A Bird's-eye View of Reranking: from List Level to Page Level

Reranking, as the final stage of multi-stage recommender systems, refines the initial lists to maximize the total utility. With the development of multimedia and user interface design, the recommendation page has evolved to a multi-list style. Separately employing traditional list-level reranking methods for different lists overlooks the inter-list interactions and the effect of different page formats, thus yielding suboptimal reranking performance. Moreover, simply applying a shared network for all the lists fails to capture the commonalities and distinctions in user behaviors on different lists. To this end, we propose to draw a bird's-eye view of \textbf{page-level reranking} and design a novel Page-level Attentional Reranking (PAR) model. We introduce a hierarchical dual-side attention module to extract personalized intra- and inter-list interactions. A spatial-scaled attention network is devised to integrate the spatial relationship into pairwise item influences, which explicitly models the page format. The multi-gated mixture-of-experts module is further applied to capture the commonalities and differences of user behaviors between different lists. Extensive experiments on a public dataset and a proprietary dataset show that PAR significantly outperforms existing baseline models.

==> Formulation.tex <==
\section{Problem Formulation}

A page-level reranking model takes as inputs the multiple ordered initial lists on the same page generated by the previous rankers, and refines the ranking lists by considering the mutual influence between items and the impact of the page format.


Given a set of users $\mathcal{U}=\{1,2,\ldots,N_u\}$ with the associated history behavior list $H_u=[h_1^u,\ldots,h_t^u]$, a set of items $\mathcal{V}=\{1,2,\ldots,N_v\}$, and a multi-list page $\mathcal{P}=\{R_1,R_2,\dots,R_n\}$ of $n$ initial lists, the problem of the page-level reranking is to jointly rerank the $n$ lists to optimize the overall utility by considering the page-wise context. Here, $N_u$ and $N_v$ denote by the number of users, and the number of items respectively, $t$ is the maximum length of the user's history behavior list, $R_i\in \Pi_{m_i}\left(\mathcal{V}\right)$, $i=1,\ldots,n$ is the $i$-th list with $m_i$ items. Let $m$ be the maximum length of the lists on the page. Then the whole page of candidate items to be reranked can be represented by an item matrix $\mathbf{X}_{n\times m}$, where $x_{i,j}$ denotes the $j$-th item in the $i$-th list, with all lists padded to the maximum length $m$.

The utility of a page is defined by the expected sum (or weighted sum) of the click probability\footnote{The click probability could be replaced by other utility metrics like conversions, purchase, etc.} for each item on the page. 
% For example, in practice, the utility is usually the total number of clicks or the total income (the click probability weighted by the bid price).
 
%   For simplicity, we assume that all lists have the same number of candidate item, i.e., $m_1=m_2=\cdots=m_n=m$.
% Our method can be easily adapted to scenarios with variable-length lists by padding them to the same length.

% Assume there are a set of users $\mathcal{U}=\{1,2,\dots,N_u\}$, a set of items $\mathcal{V}=\{1,2,\dots,N_v\}$, and a history item list $H_u=[h_1^u,\dots,h_t^u]$ with $t$ items that each user $u$ clicked.
% A multi-list page $\mathcal{P}$ can be formulated as a set of lists with diverse formats (e.g., horizontal or vertical, posters or icons): $\mathcal{P}=\{R_1,R_2,\dots,R_n\}$, where $R_i\in \Pi_{m_i}\left(\mathcal{V}\right)$ is the $i$-th list with $m_i$ items.
% For simplicity, we assume that all lists have the same number of candidate item, i.e., $m_1=m_2=\cdots=m_n=m$.
% Our method can be easily adapted to scenarios with variable-length lists by padding them to the same length.
% Therefore, the candidate items on the page can be formulated as an item matrix $\mathbf{X}_{n\times m}$, where $x_{i,j}$ denotes the $j$-th item in the $i$-th list on the page.
% Then, we encode the page format information as a symmetric distance matrix $\mathbf{D}_{nm\times nm}$, whose element indicates the distance between the corresponding pair of items on the page. More detailed information about the item distance matrix can be found in Section~\ref{sec:spatial-scaled attention}.

% Then we can define the problem of page-level reranking as follows. For a user $u$, given her history list $H_u$, a page $\mathcal{P}$ with candidate item matrix $\mathbf{X}_{n\times m}$, and the item distance matrix $\mathbf{D}_{nm\times nm}$, the page-level reranking model aims to generate $n$ reranking lists that maximizes the overall utility and better meets the user's needs on the page.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> backupv1.tex <==
\section{Introduction}
\label{sec:intro}

In multi-stage recommender systems (MRS), reranking, as the final stage, further refines the ranking list from previous ranking stage~\cite{hron2021component}.
The goal of reranking is to maximize the total utility (e.g., sum of click rates, overall revenue, or number of clicks) of the reranked lists presented to users.
The quality of reranking has a direct impact on users' experience and satisfaction, and thus plays a crucial role in MRS.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.1522\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-a.png}
        \caption{}
        \label{fig:page format illustration a}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.1529\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-b.png}
        \caption{}
        \label{fig:page format illustration b}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.152\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-c.png}
        \caption{}
        \label{fig:page format illustration c}
    \end{subfigure}
    \caption{Illustration of different page formats from Amazon e-commercial App (left), a Netflix video streaming App (medium), and an Apple App store (right). Left: single-list page containing only one traditional vertical list. Medium: multi-list page with multiple horizontal lists stacked from top to bottom. Right: multi-list page with interleavings of vertical and horizontal lists, resulting in an ``F'' shape.}
    \label{fig:page format illustration}
\end{figure}

Existing methods~\cite{ai2018learning,pang2020setrank,pei2019personalized,ai2019learning,zhuang2018globally} mainly focus on list-level reranking, which only considers the list-wise context. However, as shown in Figure~\ref{fig:page format illustration}, with the development of multimedia and user interface (UI) design, the final recommendation page presented to the user is usually in multi-list styles~\cite{gomez2015netflix,fu2022f}. 
List-level reranking algorithms estimate reranking scores based only on the context of the target list itself. The reranked lists obtained by these strategies are suboptimal when the lists are presented on a multi-list page. 

The existence of other lists changes the user behavior pattern and leads to a different distribution of utility.
For example, as shown in Figure~\ref{fig:page format illustration b}, the ``Recommended For You'' list is optimized personally according to the user's preference. 
However, the utility (e.g., click rate, viewing time) of the reranked items can be affected by popular TV shows in the ``Trending'' list or recently released videos in the ``Just Released'' list.
An item that is closely related to some trending TV shows on the same page may have a higher reranking utility, though it is less relevant to the user's preference.
Therefore, we need to draw a bird's-eye view over the whole reranking page and develop a page-level reranking algorithm, instead of solely employing list-level reranking methods within each individual list.

% The existence of other lists, as well as the page format, may change the user behavior pattern, leading to a different distribution of utility.
% Important features are omitted if we only employ list-level reranking within each individual list separately. \ww{Explain why information from other lists is important in detail. Give examples.}

% With a bird's-eye view upon the multi-list page, we argue that reranking at page level can further improve the utility by considering fine-grained interactions across different lists. As shown in Figure~\ref{fig:illustration}, the page-level reranking aims to rerank the item within each list by considering the page-wise context (e.g., the content of other lists, the page format). 

\citet{hao2021re} are the first and currently the only work to address the page-level reranking problem. 
They propose a Deep Hierarchical Attention Network Reranking (DHANR) model to generate a shared page representation via a two-layer stacked attention network.
Then, they adopt list-level reranking algorithms in each individual list, with the shared page representation as the side information.
% The page representation is used as page-wise side information for the reranking methods in each individual list. 
Nevertheless, the existing page-level reranking method DHANR still suffers from the following three limitations.

Firstly, DHANR~\cite{hao2021re} only performs coarse-grained page modeling via a hierarchical attention network. The item features in each list are first aggregated as list vectors, and then list vectors are summarized as a unified page representation. 
Such a hierarchical architecture causes the \emph{early summarization problem}, where item features are prematurely aggregated into list vectors before inter-list item interactions. As discussed above, fine-grained item interaction across different list should be further considered in the page-level reranking to improve the final utility.

Secondly, DHANR~\cite{hao2021re} ignores the impact of the page format, which indicates the list presentation style. For instance, in Figure~\ref{fig:page format illustration b}, video items are displayed as big posters, and lists are horizontally stacked from top to bottom. In Figure~\ref{fig:page format illustration c}, the page contains interleavings of vertical and horizontal lists resulting in an ``F'' shape, with App items presented by icons and texts.
Different page formats change the interaction patterns between items across lists, leading to different utility distributions.
For example, compared with the stacked-horizontal-list page, in the F-shape page, a vertical list inserted between two consecutive horizontal lists can widen the distance between the two horizontal lists, and weaken the page-level item interactions between them.
Moreover, this weakening effect further intensifies when we increase the length of inserted vertical list, or present vertical-list items by big posters in place of small icons.
Therefore, we must consider concrete list presentation and page format instead of abstract ``list'' concept to when we move from list-level reranking to page-level reranking.

Thirdly, multiple lists are treated equally in DHANR~\cite{hao2021re}, where an identical list-level reranking method is employed for all the lists with the help of shared page representation. Nevertheless, as shown in Figure~\ref{fig:page format illustration b} and~\ref{fig:page format illustration c}, the diverse list presentation styles (e.g., vertical or horizontal lists, items displayed as posters or icons), as well as different positional placements on the page, lead to various user click strategies.
Different lists may share basic hypothesis on user behaviors (e.g., position bias, cascade hypothesis~\cite{craswell2008experimental,Guo2009CCM}), but also own their distinct user behavior patterns.
For example, in Figure~\ref{fig:page format illustration c}, the position bias is more severe in horizontal lists on mobile F-shape pages since they are constructed as carousel sliders, which reduces the chance of impression for lower-ranked items.
This motivates us to model the commonalities and differences of underlying behavior patterns towards different lists, instead of simply adopting an identical reranking estimator.

% \emph{Firstly}, the user's behavior history (e.g., recent clicks, purchases, or downloads) is not fully exploited in DHANR~\cite{hao2021re}, where users' historical behaviors are equally treated, and simply converted to general features in user profiles. The items in users' history lists make different contributions when reranking different candidate items~\cite{qin2020user,xi2022multi}. For instance, a user clicks a recommended keyboard in the reranked page mostly because she bought a laptop, rather than what kind of clothes she purchased in the past. 
% Therefore, adaptive modeling over users' behavior history is essentially needed to capture users' dynamic interests and model personalized preference during the reranking stage. \ww{Move it to the last point?}

% \emph{Thirdly}, DHANR~\cite{hao2021re} only performs coarse-grained page modeling by hierarchically aggregating the features of candidate items into a unified page representation while ignoring the difference between lists. The unified page representation is shared for all the items to assist the list-level reranking methods in each individual list. 
% However, different list positions and page layout may lead to different user behavior patterns and even conflict utility distributions.
% Such a simply unified reranking score estimation may overlook some key aspects in user behaviors across lists on the reranked page, resulting in inferior reranking performance at page level.


To address the above issues, we propose a novel model named \textbf{Page-level Attentional Reranking} (PAR) to capture the multifaceted fine-grained interactions among lists with the awareness of page-wise contexts.
We propose a \textbf{hierarchical dual-side attention} (HDS-Attn) module to capture the personalized interaction between users' behavior history and the candidate items at different lists. A shared representation that contains both the page context and history information is generated for reranking score estimation of each item.
We further design a \textbf{spatial-scaled attention} (SS-Attn) network to learn item comparison patterns across lists \ww{spatial relationship between items cross sub-lists}. The attention is numerically scaled by the spatial layout and distance between each pair of items on the page, which gives explicit modelings over the page format.
Moreover, after obtaining the personalized item-wise feature representation by HDS-Attn and SS-Attn, PAR adopts the \textbf{Multi-gated Mixture-of-Experts} (MMoE~\cite{ma2018modeling}) module to capture the commonalities and differences of user behavior patterns among different lists. 
We maintain a set of parallel expert networks to capture different aspects of behavior patterns, and apply an attentional gate for each list respectively to aggregate the expert outputs for the final reranking score estimation.

The main contributions of this paper are summarized as follows:
\begin{itemize}[leftmargin=10pt]
    \item We ?
    
    \item We propose a novel Page-level Attentional Reranking (PAR) model. We design a hierarchical dual-side attention (HDS-Attn) network for interactions between historical behaviors and page-wise candidate items, and a spatial-scaled attention (SS-Attn) network to capture the page format features. Finally, an attentional gated mixture-of-experts module is utilized to model the relationship and conflict of patterns among different lists.
    
    \item Experiment.
\end{itemize}



The F-shape page is decomposed into one vertical list with 30 items and four horizontal lists with ten items. The horizontal list is split into five vertical blocks by the vertical lists, each consisting of 6 items. First, we counted the five categories that appeared most frequently on the entire dataset. Then, we fix two positions on the page, such as position $P_1$ and $P_2$, and statistically count how the probability of items at the first position $P_1$ being clicked changes with items at the two positions being each of the five categories. As illustrated in Figure~\ref{fig:data_analysis_illustr}, we have selected five fixed positions, the first position $P_1$ and the second position $P2$ in the first horizontal list, the fifth position $P_3$ and the seventh position $P_4$ in the vertical list, and the third position $P_5$ in the second horizontal list. It's worth noting that the length of the vertical list is shrunk in Figure~\ref{fig:data_analysis_illustr} due to page limitations. These five positions form four typical pairs of position relationships, yielding the heatmaps in Figure~\ref{fig:pos12}-\ref{fig:pos15}. The symbols on the horizontal and vertical axes represent the top five most frequently appearing categories, and the color variation represents how the probability of the item being clicked at position $P_1$ changes. 

\textbf{Observation 1:} Items located within the identical list can interact with each other. Figure~\ref{fig:pos12} displays how the CTR of items placed at position $P_1$ changes when items at $P_1$ and $P_2$ belong to different categories.  It is evident that if the category of $P_1$ is fixed, the CTR of $P_1$ will vary with the category of $P_2$. Similarly, when the category of $P_2$ is determined, a variation in the category of $P_1$ also leads to a variation in the CTR, indicating that the influence of $P_2$ on $P_1$ ranges from one category to another. $P_1$ and $P_2$ are adjacent in the same horizontal row, demonstrating the interaction between the items within the same list.

\textbf{Observation 2:} There is cross-list interaction between the items on the page, and it is comparable to the intra-list interaction. Except for $P_1$ and $P_1$, all the three pairs of positions in Figure~\ref{fig:pos13}-\ref{fig:pos15} are cross-list position pairs, but the mutual influence between items is still apparent. Furthermore, the magnitude of the color change in the heatmap is an indicator of the magnitude of the change in CTR so as to reflect the magnitude of the mutual influence.  Figure~\ref{fig:pos13} presents a similar magnitude of color change to Figure~\ref{fig:pos13}, illustrating that the interaction between $P_1$ and $P_3$, not in the same list, can be comparable to the interaction between $P_1$ and $P_2$ in the same list.

\textbf{Observation 3:} The more distant the items on the page, the weaker the interaction between them. The greater the color change in the heatmap, the stronger the influence between the items, and on the contrary, the more uniform the color, the weaker the influence. $P_1$ and $P_3$ lie in separate lists but adjacent to each other, so Figure~\ref{fig:pos13} shows a similar color change to Figure~\ref{fig:pos12}, where $P_1$ and $P_2$ are also adjacent. In figure~\ref{fig:pos14}, which shows the non-adjacent $P_1$ and $P_4$, the CTR varies evenly, implying that the interaction between $P_1$ and $P_4$ has diminished. As we move to $P_5$, which is more distant from $P_1$, the colors become more uniform in Figure~\ref{fig:pos15}, except for some outliers due to the small amount of data. This indicates that as the distance increases, the interaction between the two positions becomes weaker.

We propose a hierarchical dual-side attention (HDS-Attn) to enable the automatic learning of the personalized intra- and inter-list interactions at various levels. As shown in the left part of Figure~\ref{fig:framework}, the hierarchical structure synchronously extracts four different levels of interactions including the dual-side attention, the item-level aggregation, the list-level self-attention, and the list-level aggregation. which are designed for different purposes (from bottom to top):
% \begin{enumerate}
%     \item 
% \end{enumerate}

% \begin{itemize}[leftmargin=15pt]
%     \item[(1)] \textbf{Dual-side Attention} captures the personalized interactions between the candidate items and the history items.
%     \item[(2)] \textbf{Item-level Aggregation} learns the intra-list interaction, and aggregates the item vectors into the list representations $\{l_i\}_{i=1}^n$.
%     \item[(3)] \textbf{List-level Self-attention} models the mutual influence among different lists and re-weights the list representations.
%     \item[(4)] \textbf{List-level Aggregation} further learns the inter-list interaction, and aggregates the re-weighted list representations into a shared page representation $S$.
% \end{itemize}

% At the bottom level, we apply intra-list item-level attention to capture interactions from both sides of the history list and candidate items, and generate the list representations $\{l_i\}_{i=1}^n$. 
% Then, based upon the list representation, we employ list-level attention to aggregate them into a unified page representation $S$

First, for each list $i$, the input of the bottom dual-side attention is the history embeddings $\hat{\mathbf{H}}\in\mathbb{R}^{t\times d_h}$ and the candidate embeddings $\hat{\mathbf{X}}_i\in\mathbb{R}^{m\times d_x}$.
The items in the user's history list contribute differently when reranking different candidate items~\cite{xi2022multi,qin2020user}. The dual-side attention is designed to capture the different interaction effects between different history and candidate items. We maintains an affinity matrix $\mathbf{W_a}\in\mathbb{R}^{d_h \times d_x}$ to learn the importance of the association between each pair of items from both sides:
\begin{equation}
\begin{split}
    \mathbf{C}_i&=\tanh{(\hat{\mathbf{H}}\mathbf{W}_{a}\hat{\mathbf{X}}_i^\top )}\,, \\
    \mathbf{A}_i^x&=\operatorname{Softmax}\left(\tanh{(\hat{\mathbf{X}}_i\mathbf{W}_x+(\hat{\mathbf{H}}\mathbf{W}_h)^\top \mathbf{C})}\right),\\
    \mathbf{A}_i^h&=\operatorname{Softmax}\left(\tanh{(\hat{\mathbf{H}}\mathbf{W}_h + \mathbf{C}(\hat{\mathbf{X}}_i\mathbf{W}_x))}\right),\\
    % \mathbf{Q}_S&=\tanh{(\hat{\mathbf{X}}_i\mathbf{W}_x+(\hat{\mathbf{H}}\mathbf{W}_h)^\top \mathbf{C})},\\
    % \mathbf{Q}_H&=\tanh{(\hat{\mathbf{H}}\mathbf{W}_h + \mathbf{C}(\hat{\mathbf{X}}_i\mathbf{W}_x))}, \\
    % \mathbf{A}_i^x&=\text{softmax}(\mathbf{Q}_S),\\
    % \mathbf{A}_i^h&=\text{softmax}(\mathbf{Q}_H^\top )
    \Tilde{\mathbf{X}}_i&=\mathbf{A}_i^x\hat{\mathbf{X}}_i,\;\;\;\;\;\Tilde{\mathbf{H}}_i=(\mathbf{A}_i^h)^\top \hat{\mathbf{H}},
    % \Tilde{\mathbf{X}}_i&=\mathbf{A}_i^x\hat{\mathbf{X}}_i,\\
    % \Tilde{\mathbf{H}}_i&=(\mathbf{A}_i^h)^\top \hat{\mathbf{H}},
\end{split}
\label{eq:dual-side attention}
\end{equation}
where $\mathbf{W}_x\in\mathbb{R}^{d_x\times m}, \mathbf{W}_h\in\mathbb{R}^{d_h\times m}$ are learnable weight matrices. 
Attention weight matrices $\mathbf{A}_i^x\in\mathbb{R}^{m\times m}$ and $\mathbf{A}_i^h\in\mathbb{R}^{t \times m}$ are the attention probabilities of items in the candidate list and history list. 
$\Tilde{\mathbf{X}}_i=[\Tilde{\mathbf{x}}_{i,j}]_{j=1}^m\in\mathbb{R}^{m\times d_x}$ and $\Tilde{\mathbf{H}}_i=[\Tilde{\mathbf{h}}_{i,j}]_{j=1}^m\in\mathbb{R}^{m\times d_h}$ are the interacted representation matrices containing useful information from both the candidate list $i$ \xx{use $R_i$?} and history list $H_u$. 

%  \begin{equation}
%     % \begin{split}
%     \hat{\mathbf{X}}_i=\mathbf{A}_S\hat{\mathbf{X}}\, ,\,\, \hat{\mathbf{H}}=\mathbf{A}_H\hat{\mathbf{H}}\, ,\\
%     % \end{split}
%     \label{eq:att2}
%  \end{equation}
%  where $\hat{\hat{\mathbf{X}}}=\{\hat{\mathbf{x}}_1, \hat{\mathbf{x}}_2,...,\hat{\mathbf{x}}_n\}$ and $\hat{\mathbf{H}}=\{\hat{\mathbf{h}}_1, \hat{\mathbf{h}}_2,...,\hat{\mathbf{h}}_n\}$ are the interacted representation matrices containing useful information from both candidate set and history list. 

Then, we apply item-level aggregation to learn the intra-list interaction and generate the list representations.
Since not all the items contribute equally to the representation of the target list $i$, we adopt the attention mechanism to obtain the list representation $l_i$ from intra-list items following \cite{yang-etal-2016-hierarchical}:
\begin{equation}
\begin{split}
    u_{i,j} &= \tanh{(\mathbf{W}_l[\Tilde{\mathbf{x}}_{i,j} \,\Vert\, \Tilde{\mathbf{h}}_{i,j}] + b_l)},\\
    % \alpha_{i,j}& =\frac{\text{exp}(u_{i,j}^\top  q_{\text{item}})}{\sum_{k=1}^{m} \text{exp}(u_{i,j}^\top q_{\text{item}})},\\
    \alpha_{i,j}& =\operatorname{Softmax}_k(u_{i,k}^\top  q_{\text{item}}),\,j=1,\dots,m,\\
    l_i& =\sum\nolimits_{j=1}^m{\alpha_{i,j}[\Tilde{\mathbf{x}}_{i,j} \,\Vert\, \Tilde{\mathbf{h}}_{i,j}]},\\
\end{split}
\end{equation}
where $\Vert$ denotes the vector concatenation.
We feed item representations through a linear layer to get $u_{i,j}$ for each item $x_{i,j}$, and then measure the importance of the item via the similarity of the item with a trainable item-level query vector $q_{\text{item}}\in\mathbb{R}^{d_l},\,d_l=d_x+d_h$. Next, we normalize the weights $\alpha_{i,j}$ and compute the list representations $L=[l_i]_{i=1}^n\in\mathbb{R}^{n\times d_l}$. 

Next, we consider the mutual inter-list influence among different lists through the list-level self-attention layer:
\begin{equation}
    \Tilde{\mathbf{L}}=\text{Softmax}\left(\frac{\mathbf{L}\mathbf{L}^\top}{\sqrt{d_l}}\right)\mathbf{L}\,,
\end{equation}
where $\Tilde{\mathbf{L}}=[\Tilde{l}_i]_{i=1}^n \in \mathbb R^{n\times d_l}$ is the re-weighted list representation matrix, and $\sqrt{d_l}$ is used to stabilize gradients during training.

% Through the bottom dual-side attention, we obtain the list representations $L=\{l_i\}_{i=1}^n$, which already contains the weighted interactions from both candidate intra-list items and history items. Then we apply the top list-level attention to further aggregate the list vectors into a shared page representation $S$:
% \begin{equation}
%  S=\text{Attention}(\mathbf{L})=\text{softmax}\left(\frac{\mathbf{L}\mathbf{L}^\top}{\sqrt{d_l}}\right)\mathbf{L}\,,
% \end{equation}
% where $\mathbf{P}\in \mathbb R^{k\times d_l}$ is the attended matrix, and $\sqrt{d_l}$ is used to stabilize gradients during training. We denote the $i$-th row of matrix $\mathbf{P}$ as $\mathbf{p}_i$, the list embedding for list $i$.
  
%   get page representation, similar to list representation
Finally, based on the re-weighted list representations $\Tilde{\mathbf{L}}$, we employ the list-level aggregation layer to further learn the inter-list interaction and generate the unified page representation $S$. Similar to the item-level aggregation, after a linear transformation,  we maintain a learnable list-level query vector $q_{\text{list}}\in\mathbb{R}^{d_l}$ for attention weight calculation, and finally aggregate the re-weighted list representations $\Tilde{\textbf{L}}$ into a shared page representation $S$:
\begin{equation}
\begin{split}
    v_i& = \tanh{(W_p \Tilde{l}_i + b_p)}\\
    \beta_i& =\operatorname{Softmax}_i(v_i^\top q_{\text{list}}),\;i=1,\dots,n,\\
    % \beta_i& =\frac{\text{exp}(v_i^\top c_p)}{\sum_k \text{exp}(v_i^\top c_p)}\\
    S& =\sum\nolimits_{i=1}^n{\beta_i \Tilde{l}_i}\\
\end{split}
\end{equation}
% one-layer MLP + list level context vector $c_p\in\mathbb{R}^{d_l}$(randomly initialized and jointly learned during the training process)

\subsubsection{Spatial-scaled Attention}
\label{sec:spatial-scaled attention}

The SS-Attn module models the pairwise item interaction by considering the page format. As discussed in Section~\ref{sect:data_analysis}, the mutual influence between items shows negative correlation with the distance between items, which directly reflects the page format effect. We reshape the candidate item matrix $\hat{\mathbf{X}}\in \mathbb{R}^{n\times m \times d_x}$ as $\Bar{\mathbf{X}}\in \mathbb{R}^{nm\times d_x}$, where each row $\Bar{x}_{p}\,(p=1,\dots,nm)$ of the matrix $\Bar{\mathbf{X}}$ is the feature vector of a candidate item. Then we define a symmetric distance matrix $\mathbf{D}_{nm \times nm}$, whose element $d_{p,q}$ indicates the geometric distance between the corresponding pair of items on the page. In this work, we adopt the Manhattan distance to build the distance matrix. 
For example, in Figure~\ref{fig:data_analysis_illustr}, the Manhattan distances from $P_1$ to $P_i\,(i=2,3,4,5,6)$ are $1$, $2$, $1$, $2$, $5$, respectively.
It is worth noting that the distance matrix can be customized according to the page formats in different page-level reranking scenarios, or with other distance measurements (e.g., Euclidean distance, slot counting), which suggests the flexibility of our proposed model.

The SS-Attn module takes as inputs the reshaped item matrix $\Bar{\mathbf{X}}$ and the distance matrix $\mathbf{D}$, and performs multi-head self-attention on each pair of items:
\begin{equation}
\begin{split}
    \mathbf{Q}^{(b)},\mathbf{K}^{(b)},\mathbf{V}^{(b)}&=\Bar{\mathbf{X}}W_Q^{(b)},\Bar{\mathbf{X}}W_K^{(b)},\Bar{\mathbf{X}}W_V^{(b)},\;b=1,\dots,B,\\
    \mathbf{O}^{(b)}&=\operatorname{Softmax}\left(\frac{\mathbf{Q}^{(b)}\mathbf{K}^{(b)\top}}{\sqrt{d_a}}\right)\mathbf{V}^{(b)},\\
\end{split}
\end{equation}
where $B$ is the number of heads, $d_a$ is the attention size, and $W_Q^{(b)}$, $W_K^{(b)}$, $W_V^{(b)}$ are trainable matrices. 

However, the self-attention mechanism above treats each item pair equally. 
We will further scale the attention weights according to the distance matrix, which emulates the negative correlation between distances and interactions. That is, the attention weight for an item pair $(p,q)$ should be shrunk if the distance $d_{p,q}$ increases. We design the function for the scaling coefficient $\hat{d}_{p,q}$ as:
\begin{equation}
    \hat{d}_{p,q}^{(b)}=f(d_{p,q}|v^{(b)})=\frac{1+\exp(v^{(b)})}{1+\exp(v^{(b)} + 0.1 \times d_{p,q})}.
\end{equation}
$f(d_{p,q}|v)$ is a monotonically decreasing function with the value range of $(0, 1]$, and satisfies $f(0|v)=1$ and $f(+\infty|v)=0$. This means that the scaling coefficient $\hat{d}_{p,q}$ gradually decreases from $1$ to $0$ as the distance between item $p$ and $q$ grows.
The scalar $0.1$ multiplied by $d_{p,q}$ is used to re-scale the raw distance and stabilize the training.
The scalar $v^{(b)}$ is a learnable parameter that adjusts the strength of the negative correlation between distances and interactions. The larger the $v^{(b)}$ is, the steeper the function curve is, indicating a stronger negative correlation. Moreover, we maintain distinct parameters $v^{(b)}$ for different attention heads to learn different level of negative correlation effects. 

Then, we form the coefficients $\hat{d}_{p,q}$ as a matrix $\hat{\mathbf{D}}_{nm \times nm}$, and numerically scale the attention weights $\mathbf{Q}^{(b)}\mathbf{K}^{(b)\top}$:
\begin{equation}
\begin{split}
    \Bar{\mathbf{O}}^{(b)}&=\operatorname{Softmax}\left(\frac{\operatorname{ReLU}(\mathbf{Q}^{(b)}\mathbf{K}^{(b)\top})\odot \hat{\mathbf{D}}}{\sqrt{d_a}}\right)\mathbf{V}^{(b)},
\end{split}
\end{equation}
where $\odot$ is the element-wise product. Note that we employ ReLU activation to avoid negative attention weights. 
The scaling of a coefficient $\hat{d}_{p,q} \in (0, 1)$ over a negative attention weight will be inverted (i.e., amplification instead of shrinkage), which violates the negative correlation between distances and interactions.

Finally, we concatenate the multi-head spatial-scaled attention outputs, and apply a linear transformation to get the pairwise interaction matrix $\Bar{\mathbf{O}}_{nm\times d_o}$:
\begin{equation}
\begin{split}
    \Bar{\mathbf{O}} &= \left[\Bar{\mathbf{O}}^{(1)}\,\Vert\,\dots\,\Vert\,\Bar{\mathbf{O}}^{(B)}\right]\mathbf{W}_O,
\end{split}
\end{equation}
where $d_o$ is the attention output size. We reshape the matrix $\Bar{\mathcal{O}}_{nm \times d_o}$ back to $\mathbf{O}_{n \times m \times d_o}$, where the vector $o_{i,j} \in \mathbb{R}^{d_o}$ denotes the pairwise interaction vector for the $j$-th item in the $i$-th list.

% Thirdly, user behaviors on different lists have commonalities and distinctions. For one thing, user behaviors across lists may share some basic patterns (e.g., position bias, cascade hypothesis~\cite{craswell2008experimental,Guo2009CCM}) and underlying personal preferences. Collaboratively putting multiple lists together benefits the understanding of the underlying common behaviors for each user. For another, due to the theme and the format of each list, user behaviors also possess distinctions for different lists. For example, in Figure~\ref{fig:page format illustration c}, the position bias could be more severe for horizontal lists than that for vertical ones. The horizontal lists are organized by carousel sliders, which reduces the impression opportunity for lower-ranked items. Simply using the same network for all the lists may be inferior as the list-specific information is not well captured, especially for low-resource or sparse reranking lists. 

% We further design a \textbf{spatial-scaled attention} (SS-Attn) network to encapsulate the spatial relationship between items across lists. The attention is numerically scaled by the spatial layout and distance between each pair of items on the page, which provides explicit modelings over the page format.


\subsubsection{Dense Network}

In addition to the HDS-Attn and SS-Attn, the dense network is a simple fully-connected network, which is designed to capture the implicit feature interactions within each item. We feed each item embedding $\hat{x}_{i,j}$ into a shared MLP to obtain the dense feature $r_{i,j}$ for the latter reranking score estimation:
\begin{equation}
    r_{i,j}=\operatorname{MLP}(\hat{x}_{i,j}).
\end{equation}

\subsection{Reranking Score Estimation}

For the user $u$ and an initial page $\mathcal{P}$, the reranking score estimation computes the reranking score $\hat{y}_{i,j}$ for each candidate item $x_{i,j}$.
After the feature interaction \& extraction stage, we obtain the shared page representation $S$, the pairwise item interaction $o_{i,j}$, and the dense feature $r_{i,j}$.
Since user behaviors on different lists have commonalities (e.g., basic cascade hypothesis) and distinctions (e.g., different impression opportunities), we applies  the Multi-gated Mixture-of-Experts (MMoE~\cite{ma2018modeling}) module on top of the concatenation of outputs from the feature interaction \& extraction stage.

As shown in Figure~\ref{fig:framework}, there are $E$ parallel expert networks $\{e_k(\cdot)\}_{k=1}^{E}$, which are all MLPs with ReLU activations, to capture different aspects of behavior patterns. 
For each list $i$, we maintain a separate fully-connected gating network $g_i(\cdot)$ to learn a linear combination of the expert outputs. 
We feed the combined feature vector $\hat{z}_{i,j}$ into a list-specific tower network $t_i(\cdot)$ to get the final reranking score $\hat{y}_{i,j}$.
\begin{equation}
\begin{split}
    z_{i,j} &= [S \,\Vert\, r_{i,j} \,\Vert\, o_{i,j}],\\
    \gamma_{i,j,k} &=\operatorname{Softmax}_k(g_i(z_{i,j})),\;k=1,\dots,E,\\
    \hat{z}_{i,j}&=\sum\nolimits_{k=1}^{E} \gamma_{i,j,k} \times e_k(z_{i,j}),\\
    \hat{y}_{i,j} &= t_i(\hat{z}_{i,j}). \\
\end{split}
\end{equation}

The final rerankings, can be achieved by sorting the items in each list $i$ according to the estimated scores $\hat{y}_{i,j},\,j=1,\dots,m$. Given the click label matrix $\mathbf{Y}_{n\times m}$ where $y_{i,j}$ denotes the click signal for the $j$-th item in the $i$-th list, we optimize the model via binary cross-entropy loss function:
\begin{equation}
    \mathcal{L}=\sum_{u \in \mathcal{U}}\sum_{\mathcal{P}\in \mathcal{P}_u}\sum_{i=1}^n\sum_{j=1}^m y_{i,j}\log \hat{y}_{i,j} + (1-y_{i,j})\log(1-\hat{y}_{i,j})
\end{equation}


According to the input and context, the reranking methods can be divided into (\romannumeral1) list-level reranking, and (\romannumeral2) page-level reranking.

The list-level reranking methods~\cite{feng2021grn,xi2021context} take as inputs the whole lists given by the initial ranker, and emphasize the mutual influence between items. 
According to the mechanism they adopt, these methods can be roughly classified into three categories: RNN-based~\cite{ai2018learning,bello2018seq2slate,feng2021revisit}, Transformer-based~\cite{pang2020setrank,pei2019personalized}, and GNN-based~\cite{liu2020personalized} methods.
For instance, DLCM~\cite{ai2018learning} employs the gated recurrent unit (GRU)~\cite{chung2014empirical} to encode the whole ranking list into the item representations. 
% Seq2Slate~\cite{bello2018seq2slate} utilizes the pointer network with a decoder to generate the reranked list directly. 
PFRN~\cite{huang2020personalized} uses self-attention to model the context-aware information and conducts personalized flight itinerary reranking. 
The GNN-based model IRGPR~\cite{liu2020personalized} explicitly captures item interaction patterns by aggregating relational information from neighborhoods. 
MIDNN~\cite{zhuang2018globally} utilizes global feature extension and DNN to incorporate mutual influences into the feature of each item.
GSF~\cite{ai2019learning} adopts the DNN architecture to learn multivariate scoring functions by enumerating all feasible permutations of a given size.

The performance of list-level reranking algorithms is usually suboptimal when the page presented to the user is in a multi-list style.
The page-level reranking methods aim to rerank items in each list by considering the page-wise context (e.g., the content of other lists, the page format).
DHANR~\cite{hao2021re} is the first and currently the only work to address the page-level reranking problem. It designs a two-layer hierarchical attention network to progressively aggregate the item features into an unified page representation. Then, it applies an identical list-level reranking algorithm for all the lists with the page representation as shared side information.
Our proposed PAR can better model the page-wise contexts and capture fine-grained item interactions across lists, resulting in the state-of-art performance for page-level reranking.

\subsection{Whole-page Optimization}

There exist works that focus on whole-page optimization (i.e., page-level optmization), which generally fails into two categories.

The first one~\cite{wang2016beyond,wang2018optimizing,hill2017efficient,wang2017efficient,xiao2022tile,zhao2018deep,oosterhuis2018ranking} aims to find the optimal content and presentation format for each widget in the page. 
The widget does not necessarily be constructed in list format (e.g., button, image, text, list of URL). Therefore, they reduce the whole-page optimization to a combinatorial optimization problem, where graph matching~\cite{wang2016beyond,wang2018optimizing}, bandit~\cite{hill2017efficient,wang2017efficient} or reinforcement learning (RL)~\cite{xiao2022tile,zhao2018deep,oosterhuis2018ranking} algorithms are proposed. 
However, these methods are unsuitable for page-level reranking by regarding each list as a widget due to the following reasons. 
(1) They requires each widget to have limited number of variants. One list that contains $m$ items can have $m!$ variants, causing the combinatorial explosion problem.
(2) Most of these methods are online algorithms, and requires real-time interaction with users. This violates the offline paradigm in the traditional reranking setting where we seek to construct the reranker offline to avoid hurting the user experience.



The second one~\cite{gomez2015netflix,bendada2020carousel,ding2019whole,lo2021page} focuses on the problem of whole-page optimization by selecting and ranking the widgets. Each widget is constructed in a list format. Nevertheless, they does not rerank the items in each widget list (i.e., the content of the widget is fixed). Hence, they reduce the whole-page optimization to a widget-ranking problem, where we can simply adopt traditional list-level reranking algorithms by regarding each widget as a large ``item''. These methods are incompatible with the page-level reranking problem, where we seek to arrange fine-grained reranking of items within each widget. 

In this work, we focus on the page-level reranking, which is fairly different from previous whole-page optimization methods mentioned above. The goal of page-level reranking is to rerank the item within each list by considering the page-wise context (e.g., the content of other lists, the page format). 


\subsection{Multi-scenario Learning to Rank}

Multi-scenario learning to rank applies ranking services for different lists in multiple scenarios.  The adopted techniques can be generally classified into two categories: (1) multi-task learning (MTL)~\cite{chen2020scenario,li2020improving,gu2021self,sheng2021one,zhao2019recommending}, and (2) multi-agent reinforcement learning (MARL)~\cite{feng2018learning,he2020learning}.
MTL-based methods formulate the ranking problems in different scenarios as individual tasks or multiple domains. 
For example, HMoE~\cite{li2020improving} utilizes Multi-task Mixture-of-Experts~\cite{ma2018modeling,zhao2019recommending} to implicitly identify the commonalities and distinctions between scenarios. STAR~\cite{sheng2021one} designs a topologically shared model structure for ranking services in different domain scenarios. 
Compared with MTL-based methods, MARL-based algorithms requires online learning, and the decentralized agent rankers for various scenarios are not trained simultaneously.

Although we need to provide ranking services for multiple lists in different scenarios, these lists are not presented on one page in the same time. 
That is, multi-scenario recommendation is not aware of the ``page'' context, and neglects the rich page-wise information in the page-level reranking.
Conversely, in the page-level reranking, we aim to constructed a centralized reranker for multiple lists that are simultaneously displayed on the same page. Therefore, the page-wise context information (e.g., page format, item interactions across lists) should be further considered.


\section{Experiment}
\label{sec:exp}
In this section, we first compare our proposed PAR with the state-of-the-art baselines on a public dataset and a proprietary dataset. Then, we further investigate the impact of several critical components and conduct a case study to study how spatial-scaled attention models pairwise item interaction by considering the page format.
\subsection{Experiment Settings}
\subsubsection{Datasets}\label{sec:dataset} To study the effectiveness of PAR, we conduct experiments on a public dataset, Cloud Theme Click Dataset\footnote{https://tianchi.aliyun.com/dataset/dataDetail?dataId=9716}, and a proprietary dataset, AppStore.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{Cloud Theme Click Dataset}~\cite{du2019sequential} (\textbf{CTC} for short) records the click data of Cloud Theme, an important recommendation procedure in Taobao app, with different themes corresponding to varying purchase scenarios, e.g., "what to take when traveling". The dataset includes 1, 423, 835 clicks records from 355 different themes during a 6-day promotion season, the one-month purchase history of users (about 4, 294, 000 records) before the promotion started,  the item pool of each theme, and the 128-dimension embedding of 720, 210 users and 1, 361, 672 items. 
    \item \textbf{AppStore} is collected from a mainstream commercial App Store, from October 16, 2021 to November 1, 2021.  The dataset contains 394, 046 queries and 1646 items (Apps). Each App has 32 features (e.g., App developer and App category). Each page is in the form of F-shape with one vertical list inserted by four horizontal lists, and each user has a history of behavior collected in real-time, like clicks and downloads.
\end{itemize}

\subsubsection{Page and click generation}\label{page_click} As there is no publicly available dataset with page data, we use the click logs of the public CTC dataset to construct the pages where four lists are horizontally stacked from top to bottom. First, users who have clicked on less than 3 themes are filtered out. Then, for each remaining user, we construct several pages where 4 cloud themes users have clicked on are randomly sampled as the themes of 4 lists. If less than 4 themes are clicked, we negatively sample from all themes to reach a total of 4 themes. Each list has 10 items, consisting of 3 positive samples from the clicks under the list theme and 7 negative samples from all items under the list theme. After the generation of pages, we train four different DNN models on different lists of pages as our initial ranker to generate the initial rankings. 

As we generate new pages, synthetic click data is necessary to use an oracle click model to simulate user click behavior on the pages. Thus, we mainly follow Seq2Slate \cite{bello2018seq2slate} to decompose the click probability of an item into the product of relevance, position decaying, and dissimilarity probability. Firstly, we use the original click label of item $i$ as relevance probability $rel(i)$ (click: $rel(i) = 1$, non-click: $rel(i) = 0$). Secondly, a user observes item $i$ which lies in the $row(i)$-th row and $col(i)$-th column with a position decaying probability $(\frac{1}{col(i)})^{\eta_1}\cdot(\frac{1}{row(i)})^{\eta_2}$, where $\eta_1$ and $\eta_2$ are the horizontal and vertical decay parameters. Here we set $\eta_1$ and $\eta_2$ to 0.4 and 0.5. Then, when observing an item, the user will tend to click the item dissimilar to its surrounding items. 
Here, we adopt similarity probability to introduce high-order interaction between items in different lists. Items with a Manhattan distance of 1 from the current browsing item are regarded as neighbors. Then, we average the embedding of the neighbors and calculate the cosine similarity between the currently browsing item and the average embedding. One minus cosine similarity serves as the dissimilarity probability. Finally, the click probability is the product of relevance, position decaying, and dissimilarity probability. After the generation of clicks, all baselines and our model PAR are trained based on the synthetic click data.

\subsubsection{Baselines} 
% We compare our proposed PAR with the state-of-the-art page-level baselines, including page-level reranking model \textbf{DHANR}, multi-scenario LTR model \textbf{HMoE} and whole-page optimization work \textbf{TRNN}.
Since currently there is only one work, \textbf{DHANR}, that focuses on page-level reranking, we modify some models in related fields that can make use of page-level information as our baseline, such as \textbf{HMoE} in multi-scenario, \textbf{TRNN} in whole-page optimization. Besides, we also design \textbf{GlobAtt} to directly model the interactions between items on a page.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{DHANR}~\cite{hao2021re} applies a two-layer hierarchical attention network to progressively aggregate the item features into a unified page representation as shared side information to help the list-level reranking in each list.
    \item \textbf{HMoE}~\cite{li2020improving} takes advantage of Multi-task Mixture-of-Experts to implicitly identify distinctions and commonalities between lists in the feature space.
    \item \textbf{TRNN}~\cite{lo2021page} focuses on whole-page optimization and rank the widgets by a two-stage RNN. We make some modifications to TRNN so that it can employ the page information obtained by RNN to help rerank the items in different lists.
    \item \textbf{GlobAtt} adopts global multi-head self-attention, which takes as input the item feature and location, e.i., list and position, to model the interaction between any pairs of items on the page.  
\end{itemize}
% Since there are few page-level reranking models, 
We also extend the list-level reranking approaches to page-level and train separate listwise models for different lists on the page.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{miDNN}~\cite{zhuang2018globally} use global feature extension to extract mutual influence between items in the ranking lists.
    \item \textbf{GSF}~\cite{ai2019learning} employs DNN to learn multivariate scoring functions, where scores are determined jointly by multiple items in the list.
    \item \textbf{DLCM}~\cite{ai2018learning} is the first work to apply GRU to encode and rerank the top results in the ranking lists.
    \item \textbf{PRM}~\cite{pei2019personalized} models the mutual influence between any pairs of items and users' preferences by self-attention.
    \item \textbf{SetRank}~\cite{pang2020setrank} learns permutation-equivariant representations for the inputted documents via self-attention.
\end{itemize}


\subsubsection{Evaluation metrics} All the reranking models are evaluated in terms of relevance-based and utility-based metrics. For relevance-based metrics, we adopt widely-used \textit{MAP} and \textit{nDCG}~\cite{ndcg} following previous work \cite{lo2021page,pei2019personalized, ai2018learning}. Despite that there are multiple lists on the page, we calculate \textit{nDCG} and \textit{MAP} for each list and employ their average as \textit{nDCG} and \textit{MAP} of the whole page.
% Since the horizontal and vertical lists have different lengths on F-shape pages of AppStore, we calculate \textit{NDCG\_h} and \textit{MAP\_h} for the horizontal lists ,and \textit{NDCG\_v} and \textit{MAP\_v} for the vertical lists. 
As for utility-based metrics, we employ \textit{Util}, the average number of clicks on the page, and \textit{CTR}, the click probability per page, following~\cite{xi2021context}. Besides, we also compute the average click probability on each list, such as $CTR_v$, the average click probability on vertical lists, and $CTR_{h1}$, the average click probability on the first horizontal lists. The click probabilities and clicks on the public CTC dataset are generated by the same oracle click model used in \ref{page_click}. The AppStore dataset records real user clicks on the F-shape page, unlike the CTC dataset, which has an oracle click model, so we use FSCM~\cite{fu2022f}, a click model on the F-shape page, to generate click simulation on the reranked pages.

\subsubsection{Reproducibility}
The implementation of our model is publicly available\footnote{Our code is available at https://anonymous.4open.science/r/PAR-CDCE}. We adopt Adam \cite{adam} as optimizer. On the CTC dataset, there are four horizontal lists on the page with each list having a length of 10, and the maximum length of user behavior sequences for each user is 10. The learning rate is selected from $\{1\times10^{-4}, 2\times10^{-4}\}$, and the parameter of L2-Regularization from $\{1\times 10^{-4}, 2\times 10^{-4}\}$ with grid search. The batch size and the embedding size of the categorical feature are set to 128 and 16. The number of experts and the architecture of experts and towers in MMoE are 12, [200, 80], and [80]. To ensure a fair comparison, we also fine-tune all  baseline models to achieve their best performance.  

\subsection{Overall Performance}
The overall performance of our proposed PAR and baselines on the AppStore and CTC datasets are reported in Table \ref{tab:overall}, from which we have the following observations.

 First, our model PAR performs significantly better than all the baselines on both datasets. Page-level methods such as HMoE, TRNN, DHANR, and GlobAtt usually work better than list-level methods such as PRM and DLCM due to their utilization of page-level information; however, these methods are still less effective than our proposed PAR. As presented in Table~\ref{tab:overall}, PAR significantly and consistently outperforms the state-of-the-art approaches with respect to both utility-based metrics \textit{Utility} and \textit{CTR} and relevance-based metrics \textit{NDCG} and \textit{MAP} on CTC dataset. For instance, PAR improves over the best baseline with respect to \textit{Utility}, \textit{CTR}, \textit{NDCG}, and \textit{MAP} by 1.756\%, 2.232\%, 3.075\%, and 5.638\%, respectively. On AppStore dataset, PAR also achieves 6.432\% and 4.217\% improvement over the best baseline in terms of \textit{Utility} and \textit{CTR}, as shown in Table~\ref{tab:overall}. This demonstrates the effectiveness of the modeling of page format and user behavior in page-level reranking. 

Secondly, the performance of the models on the AppStore and CTC datasets diverges in terms of relevance-based metrics, \textit{NDCG} and \textit{MAP}. On the CTC dataset, PAR achieves the best NDCG and MAP, but on the AppStore data, the best relevance-based metrics are achieved by the list-level reranking method, PRM or SetRank. Perhaps, this is because the labels we use to calculate the relevance-based metric are different on the two datasets. On the CTC dataset, we apply the relevance labels (the ones used in the oracle click model to calculate relevance probability), which are not affected by examination or neighbors. On the AppStore dataset, however, we can not obtain the relevance labels and have to use click labels in the log data to calculate metrics. Yet the clicks are biased, and there may be some relevant items that have not been clicked. The list-level approach may have a tendency to place clicked items first, and therefore obtain higher NDCG and MAP. In comparison, the page-level approach may combine information from multiple lists to find more relevant items that have not been clicked, and may not necessarily place clicked items first. The divergence of relevance-based metrics between the two datasets illustrates that evaluation metrics based on past clicks do not necessarily measure the model's performance in terms of relevance and utility.

Lastly, different page formats result in different click distributions. As illustrated in Table~\ref{tab:overall}, the top clicks are predominantly located on the vertical and the first horizontal lists on the F-shape pages of AppStore dataset, with items in the first horizontal list being the most likely to be clicked. On the all-row pages of CTC dataset, clicks are concentrated on the first three horizontal lists and the probability of clicking decreases with the position of the horizontal list. It is also in the above lists that PAR shows a significant increase in CTR. The later horizontal lists have fewer clicks, hence the performance of the different models appears relatively random. On the AppStore dataset, page-level baselines outperform list-level models, but sometimes this is not the case on the CTC dataset, which may also be due to the different page formats. The cross-list mutual influence on pages with an interleaved arrangement of vertical and horizontal lists may be more potent than that on pages with only horizontal lists.
% The interleaved arrangement of vertical and horizontal lists on AppStore dataset may lead to a stronger mutual influence of the cross-list.
% \begin{table*}[]
%     % \vspace{-5pt}
%     \caption{Overall performance on AppStore datasets.}
%     % \vspace{-5pt}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|ccccccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{Util} & \textbf{CTR} & \textbf{CTR\_v} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{ctr\_row4} & \textbf{col\_nDCG} & \textbf{row\_nDCG} & \textbf{col\_MAP} & \textbf{row\_MAP} \\
% \midrule
% INIT & 1.0459 & 1.0571 & 0.2896 & 0.6953 & 0.0391 & 0.0122 & 0.0098 & 0.5774 & 0.6382 & 0.4486 & 0.5237 \\
% miDNN & 1.1704 & 1.1993 & 0.3428 & 0.7588 & 0.0396 & 0.0186 & 0.0107 & 0.5950 & 0.6481 & 0.4680 & 0.5335 \\
% GSF & 1.2183 & 1.1866 & 0.3970 & 0.7505 & 0.0420 & 0.0146 & 0.0142 & 0.5730 & 0.6497 & 0.4429 & 0.5356 \\
% DLCM & 1.3218 & 1.2593 & 0.4521 & 0.8052 & 0.0361 & 0.0176 & 0.0107 & 0.5496 & 0.6418 & 0.4088 & 0.5253 \\
% PRM & 1.3438 & 1.2748 & 0.4497 & 0.8242 & 0.0430 & 0.0151 & 0.0117 & 0.5953 & \textbf{0.6516} & 0.4684 & \textbf{0.5376} \\
% SETRANK & 1.3535 & 1.2938 & 0.4863 & 0.8013 & 0.0366 & 0.0166 & 0.0127 & \textbf{0.5969} & 0.6493 & \textbf{0.4709} & 0.5351 \\
% TRNN & 1.3970 &	1.3641 &	0.5029 &	0.7899 &	0.0431 &	0.0172 &	0.0111 &	0.5904 &	0.6463 &	0.4622 &	0.5310\\
% HMoE &	1.3706 &	1.3744 &	0.5394 &	0.7661 &	0.0414 &	0.0167 &	0.0108 &	0.5935 &	0.6483 &	0.4662 &	0.5338 \\
% DNAHR & 1.4116 & 1.3872 & 0.5312 & 0.8213 & 0.0405 & 0.0107 & 0.0078 & 0.5921 & 0.6410 & 0.4640 & 0.5241 \\
% \textbf{PAR} & \textbf{1.5024*} & \textbf{1.4457*} & \textbf{0.5801*} & \textbf{0.8413*} & \textbf{0.0503} & \textbf{0.0161} & \textbf{0.0146} & 0.5910 & 0.6439 & 0.4631 & 0.5281\\
% \bottomrule
% \end{tabular}
% }
% \footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
%     \label{tab:appstore}
% \end{table*}

% \begin{table*}[]
%     \caption{Overall performance on CTC datasets.}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|cccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{utility} & \textbf{CTR} & \textbf{ctr\_row0} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{NDCG} & \textbf{MAP} \\
% \midrule
% init & 1.2706 & 1.2545 & 0.5030 & 0.3747 & 0.3161 & 0.0607 & 0.4953 & 0.3241 \\
% miDNN & 1.3530 & 1.3305 & 0.5302 & 0.3884 & 0.3439 & 0.0680 & 0.5090 & 0.3415 \\
% GSF & 1.2791 & 1.3252 & 0.5308 & 0.3899 & 0.3386 & 0.0659 & 0.5238 & 0.3618 \\
% DLCM & 1.3494 & 1.3603 & 0.5371 & 0.4064 & 0.3504 & 0.0664 & 0.5303 & 0.3692 \\
% PRM & 1.3722 & 1.3710 & 0.5474 & 0.4014 & 0.3539 & 0.0684 & 0.5212 & 0.3578 \\
% SetRank & 1.3643 & 1.3635 & 0.5432 & 0.4026 & 0.3507 & 0.0671 & 0.5300 & 0.3689 \\
% TRNN & 1.3750 & 1.3602 & 0.5533 & 0.3965 & 0.3430 & 0.0674 & 0.5220 & 0.3587 \\
% HMoE & 1.3615 & 1.3608 & 0.5452 & 0.3968 & 0.3492 & 0.0696 & 0.5236 & 0.3609 \\
% DHANR & 1.3303 & 1.3512 & 0.5382 & 0.3992 & 0.3450 & \textbf{0.0687} & 0.5233 & 0.3597 \\
% \textbf{PAR} & \textbf{1.3963*} & \textbf{1.4016*} & \textbf{0.5648*} & \textbf{0.4153*} & \textbf{0.3540} & 0.0675 & \textbf{0.5463*} & \textbf{0.3897*}\\
% % PAR	1.3963*	1.4016*	0.5648*	0.4153*	0.3540	0.0675	0.5463*	0.3897*
% \bottomrule
% \end{tabular}
% }
% \footnotesize \flushleft\hspace{3cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
% \label{tab:CloudThemeClick}
% \end{table*}

\begin{table*}[]
% \vspace{-5pt}
    \caption{Overall performance on AppStore and CTC datasets.}
    % \vspace{-5pt}
    \centering
\setlength{\tabcolsep}{2pt}
% \scalebox{0.79}{
\begin{adjustbox}{max width=1\linewidth}
\begin{tabular}{c|ccccccccc|cccccccc}
\toprule
\multirow{2}{*}{\textbf{Models}} & \multicolumn{9}{c}{\textbf{AppStore dataset}}  & \multicolumn{8}{c}{\textbf{CTC dataset}}  \\
\cmidrule{2-18}
& $\mathbf{Util}$            & $\mathbf{CTR}$             & $\mathbf{CTR_v}$          & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{CTR_{h4}}$         & $\mathbf{nDCG}$            & $\mathbf{MAP}$             & $\mathbf{Util}$            & $\mathbf{CTR}$             & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{nDCG}$             & $\mathbf{MAP}$              \\
\midrule
INIT                             & 1.0459           & 1.0571           & 0.2896           & 0.6953           & 0.0391          & 0.0122          & 0.0098          & 0.6260          & 0.5087          & 1.2706           & 1.2545           & 0.5030           & 0.3747           & 0.3161          & 0.0607          & 0.4953           & 0.3241           \\
miDNN                            & 1.1704           & 1.1993           & 0.3428           & 0.7588           & 0.0396          & \textbf{0.0186} & 0.0107          & 0.6375          & 0.5204          & 1.3530           & 1.3305           & 0.5302           & 0.3884           & 0.3439          & 0.0680          & 0.5090           & 0.3415           \\
GSF                              & 1.2183           & 1.1866           & 0.3970           & 0.7505           & 0.0420          & 0.0146          & 0.0142          & 0.6344          & 0.5171          & 1.2791           & 1.3252           & 0.5308           & 0.3899           & 0.3386          & 0.0659          & 0.5238           & 0.3618           \\
DLCM                             & 1.3218           & 1.2593           & 0.4521           & 0.8052           & 0.0361          & 0.0176          & 0.0107          & 0.6234          & 0.5020          & 1.3494           & 1.3603           & 0.5371           & 0.4064           & 0.3504          & 0.0664          & 0.5303           & 0.3692           \\
PRM                              & 1.3438           & 1.2748           & 0.4497           & 0.8242           & 0.0430          & 0.0151          & 0.0117          & \textbf{0.6403}          & \textbf{0.5238} & 1.3722           & 1.3710           & 0.5474           & 0.4014           & 0.3539          & 0.0684          & 0.5212           & 0.3578           \\
SetRank                          & 1.3535           & 1.2938           & 0.4863           & 0.8013           & 0.0366          & 0.0166          & 0.0127          & 0.6388   & 0.5223          & 1.3643           & 1.3635           & 0.5432           & 0.4026           & 0.3507          & 0.0671          & 0.5300           & 0.3689           \\
GlobAtt	& 1.3896 & 1.3611 & 0.5335 &	0.7586 &	0.0415 &	0.0169 &	0.0107 &	0.5335 &	0.7586 &	1.3678 &	1.3638 &	0.5449 & 	0.4039 &	0.3474 & 	0.0676 &	0.5185 \\
TRNN                             & 1.3970           & 1.3641           & 0.5029           & 0.7899           & 0.0431          & 0.0172          & 0.0111          & 0.6351          & 0.5172          & 1.3750           & 1.3602           & 0.5533           & 0.3965           & 0.3430          & 0.0674          & 0.5220           & 0.3587           \\
HMoE                             & 1.3706           & 1.3744           & 0.5394           & 0.7661           & 0.0414          & 0.0167          & 0.0108          & 0.6373          & 0.5203          & 1.3615           & 1.3608           & 0.5452           & 0.3968           & 0.3492          & \textbf{0.0696} & 0.5236           & 0.3609           \\
DNAHR                            & 1.4116           & 1.3872           & 0.5312           & 0.8213           & 0.0405          & 0.0107          & 0.0078          & 0.6312          & 0.5121          & 1.3303           & 1.3512           & 0.5382           & 0.3992           & 0.3450          & 0.0687          & 0.5233           & 0.3597           \\
\textbf{PAR}                     & \textbf{1.5024*} & \textbf{1.4457*} & \textbf{0.5801*} & \textbf{0.8413*} & \textbf{0.0503} & 0.0161          & \textbf{0.0146} & 0.6333          & 0.5151          & \textbf{1.3963*} & \textbf{1.4016*} & \textbf{0.5648*} & \textbf{0.4153*} & \textbf{0.3540} & 0.0675          & \textbf{0.5463*} & \textbf{0.3897*}\\
\bottomrule
\end{tabular}
\end{adjustbox}
% }

\footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
\label{tab:overall}
\end{table*}

\begin{table*}[]
% \vspace{-5pt}
    \caption{Ablation on AppStore and CTC datasets.}
    % \vspace{-5pt}
    \centering
\setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.2}
% \scalebox{0.86}{
\begin{adjustbox}{max width=1\linewidth}
\begin{tabular}{c|ccccccccc|cccccccc}
\toprule
\multirow{2}{*}{\textbf{Variants}} & \multicolumn{9}{c|}{\textbf{AppStore dataset}} & \multicolumn{8}{c}{\textbf{CTC dataset}} \\
\cmidrule{2-18}
& $\mathbf{Util}$            & $\mathbf{CTR}$             & $\mathbf{CTR_v}$          & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{CTR_{h4}}$         & $\mathbf{nDCG}$            & $\mathbf{MAP}$             & $\mathbf{Util}$            & $\mathbf{CTR}$             & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{nDCG}$             & $\mathbf{MAP}$              \\
\midrule
PAR-HDSA                           & 1.4482          & 1.4236          & 0.5515          & 0.8009          & 0.0432          & 0.0171          & 0.0110          & 0.6292          & 0.5097          & 1.3594          & 1.3712          & 0.5621          & 0.4065          & 0.3399          & 0.0627          & 0.5271           & 0.3648           \\
PAR-MMoE                           & 1.3950          & 1.4203          & 0.5501          & 0.7997          & 0.0427          & 0.0169          & 0.0108          & \textbf{0.6349}          & \textbf{0.5171} & 1.3821          & 1.3825          & 0.5566          & 0.4106          & 0.3519          & 0.0634          & 0.5321           & 0.3722           \\
PAR-SSA                            & 1.4595          & 1.4338          & 0.5570          & 0.8083          & 0.0414          & 0.0165          & 0.0105          & 0.6328 & 0.5143          & 1.3757          & 1.3718          & 0.5502          & 0.3978          & \textbf{0.3541} & \textbf{0.0698} & 0.5305           & 0.3688           \\
PAR-DN      & 1.4743          & 1.4343          & 0.5555          & 0.8076          & 0.0431          & 0.0171          & 0.0110          & 0.6327          & 0.5144          & 1.3146          & 1.3876          & 0.5547          & 0.4109          & 0.3506          & 0.0670          & 0.5378           & 0.3787           \\
PAR-scale                          & 1.4136          & 1.4356          & 0.5547          & 0.8091          & 0.0436          & \textbf{0.0172} & 0.0109          & 0.6305          & 0.5116          & 1.3871          & 1.3803          & 0.5537          & 0.4096          & 0.3501          & 0.0669          & 0.5367           & 0.3779           \\
\textbf{PAR}                       & \textbf{1.5024} & \textbf{1.4457} & \textbf{0.5801} & \textbf{0.8413} & \textbf{0.0503} & 0.0161          & \textbf{0.0146} & 0.6333          & 0.5151          & \textbf{1.3963} & \textbf{1.4016} & \textbf{0.5648} & \textbf{0.4153} & 0.3540          & 0.0675          & \textbf{0.5463*} & \textbf{0.3897*}\\
\bottomrule
\end{tabular}
\end{adjustbox}
% }
\footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
\label{tab:ablation}
\end{table*}

% \begin{table*}[]
%     % \vspace{-5pt}
%     \caption{Ablation on AppStore dataset.}
%     % \vspace{-5pt}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|ccccccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{utility} & \textbf{CTR} & \textbf{ctr\_col} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{ctr\_row4} & \textbf{col\_NDCG} & \textbf{row\_NDCG} & \textbf{col\_MAP} & \textbf{row\_MAP} \\
% \midrule
% PAR-HDSA             & 1.4482           & 1.4236          & 0.5515            & 0.8009             & 0.0432             & 0.0171    & 0.0110             & 0.5843             & 0.6404             & 0.4544            & 0.5235            \\
% PAR-MMoE             & 1.3950           & 1.4203          & 0.5501            & 0.7997             & 0.0427             & 0.0169             & 0.0108             & 0.5836             & \textbf{0.6477}    & 0.4531            & \textbf{0.5331}   \\
% PAR-SSA              & 1.4595           & 1.4338          & 0.5570            & 0.8083             & 0.0414    & 0.0165    & 0.0105             & \textbf{0.5914}    & 0.6431             & \textbf{0.4641}   & 0.5269            \\
% PAR-DN             & 1.4743           & 1.4343          & 0.5555            & 0.8076             & 0.0431             & 0.0171    & 0.0110             & 0.5760             & 0.6469             & 0.4432            & 0.5322            \\
% PAR-scale &	1.4136 &	1.4356 &	0.5547 &	0.8091 &	0.0436 &	\textbf{0.0172} &	0.0109 &	0.5872 &	0.6413 &	0.4586 &	0.5248 \\
% \textbf{PAR}         & \textbf{1.5024}  & \textbf{1.4457} & \textbf{0.5801}   & \textbf{0.8413}    & \textbf{0.0503}    & 0.0161             & \textbf{0.0146}    & 0.5910    & 0.6439             & 0.4631            & 0.5281           \\
% % PAR-HDSA & 1.4585 & 1.4279 & 0.5529 & 0.8035 & 0.0432 & \textbf{0.0173} & 0.011 & 0.5903 & 0.6381 & 0.4614 & 0.5205 \\
% % PAR-MMoE & 1.4053 & 1.4217 & 0.5516 & 0.8006 & 0.0421 & 0.0168 & 0.0106 & 0.5829 & \textbf{0.6504} & 0.4520 & \textbf{0.5364} \\
% % PAR-SSA & 1.4448 & 1.4314 & 0.5525 & 0.8070 & 0.0437 & 0.0172 & 0.011 & 0.5908 & 0.6442 & 0.4626 & 0.5287 \\
% % \textbf{PAR} & \textbf{1.5024} & \textbf{1.4457} & \textbf{0.5801} & \textbf{0.8413} & \textbf{0.0503} & 0.0161 & \textbf{0.0146} & \textbf{0.5910} & 0.6439 & \textbf{0.4631} & 0.5281\\
% \bottomrule
% \end{tabular}
% }
% % \footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
%     \label{tab:ablation_appstore}
% \end{table*}

% \begin{table*}[]
%     % \vspace{-5pt}
%     \caption{Ablation on CTC dataset.}
%     % \vspace{-5pt}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|cccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{utility} & \textbf{CTR}    & \textbf{ctr\_row0} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{NDCG}    & \textbf{MAP}     \\
% \midrule
% PAR-HDSA             & 1.3594           & 1.3712          & 0.5621             & 0.4065             & 0.3399             & 0.0627             & 0.5271           & 0.3648           \\
% PAR-MMoE             & 1.3821           & 1.3825          & 0.5566             & 0.4106             & 0.3519             & 0.0634             & 0.5321           & 0.3722           \\
% PAR-SSA              & 1.3757           & 1.3718          & 0.5502             & 0.3978             & \textbf{0.3541}    & \textbf{0.0698}    & 0.5305           & 0.3688           \\
% PAR-DN             & 1.3146           & 1.3876          & 0.5547             & 0.4109             & 0.3506             & 0.0670             & 0.5378           & 0.3787           \\
% PAR-scale &	1.3871 &	1.3803 &	0.5537 &	0.4096 &	0.3501 &	0.0669 &	0.5367 &	0.3779\\
% \textbf{PAR}         & \textbf{1.3963}  & \textbf{1.4016} & \textbf{0.5648}    & \textbf{0.4153}    & 0.3540             & 0.0675             & \textbf{0.5463*} & \textbf{0.3897*}\\
% \bottomrule
% \end{tabular}
% }
% % \footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
%     \label{tab:ablation_ctc}
% \end{table*}



\subsection{In-depth Analysis}

\subsubsection{Ablation study}
To investigate the effectiveness of each component in PAR, we design several variants of PAR and conduct a series of experiments on AppStore and CTC datasets.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{PAR-HDSA} replaces the co-attention module in HDS-Attn with self-attention.
    \item \textbf{PAR-MMoE} replaces MMoE with a single MLP.
    \item \textbf{PAR-SSA} removes the SS-Attn module.
    \item \textbf{PAR-DN} removes the dense network.
    \item \textbf{PAR-scale} removes the re-scaling of the raw self-attention weights, equivalent to replacing SS-Attn with self-attention.
\end{itemize}
The comparison of above variants and the original PAR on AppStore and CTC datasets are presented in Table~\ref{tab:ablation}. Compared to the original PAR, the performances of the variants all decline to some extent, indicating the effectiveness of each module. Among all the variants, PAR-DSHA suffered almost the greatest drop in performance, which suggests that the consideration of user history and interests can facilitate the performance improvements in page-level reranking. After removing the MMoE and SSA modules, there is also a large decrease, illustrating the importance of modeling the differences and commonalities between lists and user comparison behavior. There is no significant gap between the results of PAR-SSA and PAR-scale, revealing that it is the re-scaling of attention weights that contributes primarily to the SSA module. Thus, the basic self-attention is insufficient to  model users' comparison behavior on different page formats. It is essential to design distance matrices specific to different page formats.

\subsubsection{Case Study}

 \begin{figure}[h]
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{figures/case-study.pdf}
    \caption{
    (a) The attention weights (normalized along the x-axis) of the list-level self-attention in HDS-Attn. 
    (b) The pairwise attention weights between the target item (\textcolor{red}{red box}) and other items in SS-Attn.}
    \label{fig:case_study}
\end{figure}

%  \begin{figure}[h]
%     \centering
%     \begin{minipage}[c]{0.23\textwidth}
%     \includegraphics[width=\linewidth]{figures/list-case-study.pdf}
%     \subcaption{}
%     \label{fig:list_att}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[c]{0.23\textwidth}
%     \includegraphics[width=\linewidth]{figures/Spatial-case-study.pdf}
%     \subcaption{}
%     \label{fig:spatial_att}
%     \end{minipage}
%     \caption{
%     (a) The attention weights (normalized along the x-axis) of the list-level self-attention in HDS-Attn. 
%     (b) The pairwise attention weights between the target item (\textcolor{red}{red box}) and other items in SS-Attn.}
%     \label{fig:case_study}
% \end{figure}

To explore the interaction between lists and the spatial relationship between items across the lists, we select a page from the AppStore and visualize the attention weights obtained from list-level self-attention and spatial-scaled attention. Figure~\ref{fig:case_study}(a) presents the heatmap of the vertical list $v$ and the four horizontal lists $h1$, $h2$, $h3$, and $h4$, with each row being the attention weights of a list on the horizontal axis lists. As for spatial-scaled attention, we select a target item at the third position of the second horizontal list and then visualize its attention weights on all the items on the F-shape page in Figure~\ref{fig:case_study}(b).

In Figure~\ref{fig:case_study}(a), all lists have a high attention weight for $h1$, probably because $h1$ has the most clicks and can provide more information. List $v$, neighboring all the other lists, receives the next highest number of clicks, hence the other lists also have a relatively high attention weight for $v$.  Conversely, $h2$-$h4$ which locate further away with lower CTR have smaller attention weights. From Figure~\ref{fig:case_study}(b), we can obtain two observations. First, there is a pattern of spatial decay. The target item has the greatest attention weight on itself, and the weights on its surrounding items roughly follow the pattern that the further away the item is, the less weight it gets. Second, the weights of the bottom items are usually greater than those of the top items, which is inconsistent with the common cascade assumption. This may be attributed to the fact that the item that user focuses is usually swept to the upper part of the phone screen, making it easier for the user to compare the target item with the bottom items.

% \ww{TODO: exp design, discussion}

==> backupv2.tex <==

\section{Introduction}
\label{sec:intro}

In multi-stage recommender systems (MRS), reranking, as the final stage,  re-orders the input ranking lists from the previous ranking stage by modeling the cross-item influence~\cite{hron2021component}.
The goal of reranking is to maximize the total utility (e.g., overall revenue, or the number of clicks) of the reranked lists.
The quality of reranking has a direct impact on users' experience and satisfaction, and thus plays a crucial role in MRS~\cite{liu2022neural}.

%  of the reranked lists presented to users
\begin{figure}[t]
    \centering
    \hfill
    \begin{subfigure}{0.11\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-a.png}
        \caption{}
        \label{fig:page format illustration a}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.11\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-b-2.png}
        \caption{}
        \label{fig:page format illustration b}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.11\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-c.png}
        \caption{}
        \label{fig:page format illustration c}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{figures/page-format-no-arrows-c.png}
        % \caption{}
        % \label{fig:page format illustration c}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Illustration of different page formats. Left: single vertical list in Amazon Shopping. Medium: multiple horizontal lists in Netflix. Right: multi-list page with interleavings of vertical and horizontal lists in Apple App Store.}
    \label{fig:page format illustration}
    \vspace{-15pt}
\end{figure}
%  Left: single vertical list in Amazon Shopping. Medium: multiple horizontal lists in Netflix. Right: multi-list page with interleavings of vertical and horizontal lists in Apple App Store.

% Illustration of different page formats from Amazon e-commercial App (left), Netflix video streaming App (medium), and Apple App store (right). Left: single-list page containing only one traditional vertical list. Medium: multi-list page with multiple horizontal lists stacked from top to bottom. Right: multi-list page with interleavings of vertical and horizontal lists, resulting in an ``F'' shape.

Various reranking methods~\cite{ai2018learning,pang2020setrank,pei2019personalized,ai2019learning,zhuang2018globally} have been developed in recent years, but they are mainly \textit{list-level reranking} models. List-level models rerank a single list each time, and only consider the cross-item influence within the individual list~\cite{liu2022neural}. Such a reranking strategy, though already found useful in many industrial applications, may still be suboptimal. In fact, with the development of multimedia and user interface design, the final recommendation page presented to the user is usually in a \textit{multi-list style}~\cite{gomez2015netflix,fu2022f}. As shown in Figure~\ref{fig:page format illustration}, each list on the multi-list page often highlights a particular theme (e.g., ``Trending'', ``Games''), sometimes even with a tailored layout (e.g., size, location).
% The existence of other lists changes the user behavior patterns of a single list, leading to a different utility distribution. 
The existence of other lists changes the user behavior patterns, leading to a different utility distribution. 
In this work, we propose to draw a bird's-eye view over the whole reranking page and develop a \textit{page-level reranking} algorithm. While intuitively useful to integrate page-wise information, it is nontrivial to jointly perform reranking for multiple lists with the following three major challenges (\textbf{C1} - \textbf{C3}).

\textbf{(C1)} Firstly, incorporating intra-list and inter-list interactions is essential for page-level reranking. Items from the same list are usually related to the same theme. Modeling the cross-item influence within the list (i.e., intra-list interaction) and identifying the best permutation over candidate items is the main objective for reranking~\cite{liu2022neural}. 
Moreover, we observe that the inter-list interaction is also crucial for page-level modeling --- whether a user is interested in an item is also influenced by items placed in other lists. Independent optimization for each individual list ignores the context in other lists. 
For example, in Figure~\ref{fig:page format illustration b}, the TV series \emph{Stranger Things Season 3} should have a low utility in the ``Recommended For You'' list (rank 2), suppose the user had already finished the series years ago.
However, its sequel \emph{Stranger Things Season 4} in the ``Trending'' list (rank 1) can motivate the user to re-watch the \emph{Season 3} for a second time to recall the previous story, leading to a different utility distribution.
% For example, the ``Recommended For You'' list in Figure~\ref{fig:page format illustration b} is filled with items that are most likely to be favored by the users according to their historical preferences. But its actual utility is affected by other lists (e.g., ``Trending'' or ``Just Released''). A popular item in ``Trending'' may attract more attention, and hence lower the reranking utility for some items in the ``Recommended For You'' list, even if it is less relevant to the user's preference. 
% To this end, both intra- and inter-list interactions should be considered for page-level reranking to provide a holistic view.
Thus, both intra- and inter-list interactions should be considered to provide a holistic view.

% independent optimization in one scenario only uses its own user
% data but ignores the context in other scenarios.

\textbf{(C2)} Secondly, the page format of the reranking page affects how items interact with each other, and thus should also be introduced to the page-level reranking. For instance, in Figure~\ref{fig:page format illustration b}, lists of movies and TV shows are horizontally stacked from top to bottom. In Figure~\ref{fig:page format illustration c}, the page contains interleavings of vertical and horizontal lists and forms an ``F'' shape. Compared with the page of stacked horizontal lists, the horizontal lists in the F-shape page are separated by a vertical list with a larger distance, so that the influence between items from two consecutive horizontal lists may be less. The influence becomes even less if the length or size of the inserted vertical list is increased, which further enlarges the distance between lists. We also provide evidence for such an effect in Section~\ref{sect:data_analysis}. Therefore, page-level reranking is expected to formulate the page format (e.g., the size and location of the items).

%  \begin{figure*}[h]
%     \centering
%     \begin{minipage}[c]{0.14\textwidth}
%     \includegraphics[width=\linewidth]{figures/data-analysis-illustration-3.png}
%     \subcaption{}
%     \label{fig:data_analysis_illustr}
%     \end{minipage}
%     \hspace{7pt}
%     \begin{minipage}[c]{0.19\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos12.pdf}
%     \subcaption{}
%     \label{fig:pos12}
%     \end{minipage}
%     \begin{minipage}[c]{0.19\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos13.pdf}
%     \subcaption{}
%     \label{fig:pos13}
%     \end{minipage}
%     \begin{minipage}[c]{0.19\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos14.pdf}
%     \subcaption{}
%     \label{fig:pos14}
%     \end{minipage}
%     \begin{minipage}[c]{0.23\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos15.pdf}
%     \subcaption{}
%     \label{fig:pos15}
%     \end{minipage}
%     \caption{(a) The five fixed position on the F-shape page. We shrink the length of vertical blocks due to page limitations. (b) CTR of $P_1$ as $P_2$ varies. (c) CTR of $P_1$ as $P_3$ varies. (d) CTR of $P_1$ as $P_4$ varies. (e) CTR of $P_1$ as $P_5$ varies.}
%     \label{fig:data_analysis}
% \end{figure*}

 \begin{figure*}[h]
    \vspace{-10pt}
    \centering
    \begin{minipage}[c]{0.12\textwidth}
    \includegraphics[width=\linewidth]{figures/data-analysis-illustration-6.png}
    \subcaption{}
    \label{fig:data_analysis_illustr}
    \end{minipage}
    \hspace{7pt}
    \begin{minipage}[c]{0.16\textwidth}
    \includegraphics[width=\linewidth]{figures/new_pos12.pdf}
    \subcaption{}
    \label{fig:pos12}
    \end{minipage}
    \begin{minipage}[c]{0.16\textwidth}
    \includegraphics[width=\linewidth]{figures/new_pos13.pdf}
    \subcaption{}
    \label{fig:pos13}
    \end{minipage}
    \begin{minipage}[c]{0.16\textwidth}
    \includegraphics[width=\linewidth]{figures/new_pos14.pdf}
    \subcaption{}
    \label{fig:pos14}
    \end{minipage}
    \begin{minipage}[c]{0.16\textwidth}
    \includegraphics[width=\linewidth]{figures/new_pos15.pdf}
    \subcaption{}
    \label{fig:pos15}
    \end{minipage}
    \begin{minipage}[c]{0.195\textwidth}
    \includegraphics[width=\linewidth]{figures/new_pos16.pdf}
    \subcaption{}
    \label{fig:pos16}
    \end{minipage}
    \vspace{-10pt}
    \caption{(a) The five fixed positions on the F-shape page. The red auxiliary lines and dots are provided for the illustration of the Manhattan distance measurement between items. 
    % We shrink the length of vertical blocks due to page limitations.
    (b) CTR of $P_1$ as $P_2$ varies. (c) CTR of $P_1$ as $P_3$ varies. (d) CTR of $P_1$ as $P_4$ varies. (e) CTR of $P_1$ as $P_5$ varies. (f) CTR of $P_1$ as $P_6$ varies.}
    \label{fig:data_analysis}
    \vspace{-13pt}
\end{figure*}

% Different page formats change the interaction patterns between items across lists, leading to different utility distributions.
\textbf{(C3)} Thirdly, user behaviors on different lists have commonalities and distinctions. For one thing, user behaviors across lists may share some basic patterns (e.g., position bias, cascade hypothesis~\cite{craswell2008experimental,Guo2009CCM}) and underlying personal preferences. Collaboratively putting multiple lists together benefits the understanding of the underlying common behaviors for each user. For another, due to the theme and format of each list, user behaviors also possess distinctions for different lists. For example, in Figure~\ref{fig:page format illustration c}, the position bias could be more severe for horizontal lists than that for vertical ones. The horizontal lists are designed as carousel sliders, which reduces the impression opportunity for lower-ranked items. Simply using the same network for all the lists may be inferior as the list-specific information is not well captured, especially for low-resource or sparse reranking lists. 

Although \citet{hao2021re} consider the page-level information and propose the DHANR model, they only transform the items on the page to a static page representation by a hierarchical attention network. The obtained page representation is fed into the list-level reranking model as the static side information for each individual list, unaware of the dynamic inter-list interactions between items or the page format of the whole page. Moreover, DHANR fails to capture the commonalities and distinctions among lists.


To address the above issues, we propose a novel model named \underline{P}age-level \underline{A}ttentional \underline{R}eranking (PAR) for page-level reranking. Multiple lists are jointly reranked with a unified model to capture the multifaceted fine-grained mutual influences among lists. Firstly, we propose hierarchical dual-side attention (HDS-Attn) module to extract the intra- and inter-list interactions according to users' individual behavior history \textbf{(C1)}. 
% Next, a spatial-scaled attention (SS-Attn) network is designed to encapsulate the spatial relationship between items across lists. The attention is numerically scaled by the spatial layout and distance between each pair of items on the page, which provides explicit modelings over the page format \textbf{(C2)}. 
Next, the spatial-scaled attention (SS-Attn) network is designed to encapsulate the pairwise influence between items with respect to their spatial relationship. The attention is numerically scaled by the distance between items on the page, which provides explicit modelings over the page format \textbf{(C2)}. 
Lastly, after obtaining the
% personalized item-wise
interacted feature representation from HDS-Attn and SS-Attn, PAR adopts the Multi-gated Mixture-of-Experts (MMoE~\cite{ma2018modeling}) module to capture the commonalities and differences of user behavior patterns among different lists \textbf{(C3)}. MMoE maintains a set of parallel expert networks to capture different aspects of behavior patterns, and applies an attentional gate with list-specific parameters for each individual list to aggregate the expert outputs for the final score estimation.

The main contributions of this paper are listed as follows:
\vspace{-10pt}
\begin{itemize}
    % \item We propose to draw a bird’s-eye view over the whole reranking page to jointly rerank multiple lists to optimize the overall utility by considering the page-wise information (e.g., the existence of other lists, the page format). 
    \item We propose to draw a bird’s-eye view over the whole reranking page to jointly rerank multiple lists and optimize the overall utility by considering the page-wise information. To the best of our knowledge, this is the first work to consider the effect of general page format for page-level reranking.
    \item We conduct data analysis based on a multi-list dataset, and identify the importance of intra- and inter-list interactions and the spatial relationship (i.e., reflection of page format) between items.
    \item We propose a novel Page-level Attentional Reranking (PAR) model. We design an HDS-Attn module for the personalized intra- and inter-list interactions, and an SS-Attn module to incorporate the page format. The MMOE module is equipped to capture the commonalities and distinctions for different lists.
    \item Extensive experiments on a public dataset and a proprietary dataset show that PAR achieves the state-of-the-art performance compared with existing baseline models.
\end{itemize}


% To address the above issues, we propose a novel model named \textbf{Page-level Attentional Reranking} (PAR) to capture the multifaceted fine-grained interactions among lists with the awareness of page-wise contexts.
% We propose a \textbf{hierarchical dual-side attention} (HDS-Attn) module to capture the personalized interaction between users' behavior history and the candidate items at different lists. A shared representation that contains both the page context and history information is generated for reranking score estimation of each item.
% We further design a \textbf{spatial-scaled attention} (SS-Attn) network to learn item comparison patterns across lists \ww{spatial relationship between items cross sub-lists}. The attention is numerically scaled by the spatial layout and distance between each pair of items on the page, which gives explicit modelings over the page format.
% Moreover, after obtaining the personalized item-wise feature representation by HDS-Attn and SS-Attn, PAR adopts the \textbf{Multi-gated Mixture-of-Experts} (MMoE~\cite{ma2018modeling}) module to capture the commonalities and differences of user behavior patterns among different lists. 
% We maintain a set of parallel expert networks to capture different aspects of behavior patterns, and apply an attentional gate for each list respectively to aggregate the expert outputs for the final reranking score estimation.

% The main contributions of this paper are summarized as follows:
% \begin{itemize}[leftmargin=10pt]
%     \item We ?
    
%     \item We propose a novel Page-level Attentional Reranking (PAR) model. We design a hierarchical dual-side attention (HDS-Attn) network for interactions between historical behaviors and page-wise candidate items, and a spatial-scaled attention (SS-Attn) network to capture the page format features. Finally, an attentional gated mixture-of-experts module is utilized to model the relationship and conflict of patterns among different lists.
    
%     \item Experiment.
% \end{itemize}


\section{Data Analysis}
\label{sect:data_analysis}


%  \begin{figure*}[h]
%     \centering
%     \begin{minipage}[c]{0.14\textwidth}
%     \includegraphics[width=\linewidth]{figures/data-analysis-illustration-3.png}
%     \subcaption{}
%     \label{fig:data_analysis_illustr}
%     \end{minipage}
%     \hspace{7pt}
%     \begin{minipage}[c]{0.19\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos12.pdf}
%     \subcaption{}
%     \label{fig:pos12}
%     \end{minipage}
%     \begin{minipage}[c]{0.19\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos13.pdf}
%     \subcaption{}
%     \label{fig:pos13}
%     \end{minipage}
%     \begin{minipage}[c]{0.19\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos14.pdf}
%     \subcaption{}
%     \label{fig:pos14}
%     \end{minipage}
%     \begin{minipage}[c]{0.23\textwidth}
%     \includegraphics[width=\linewidth]{figures/pos15.pdf}
%     \subcaption{}
%     \label{fig:pos15}
%     \end{minipage}
%     \caption{(a) The five fixed position on the F-shape page. We shrink the length of vertical blocks due to page limitations. (b) CTR of $P_1$ as $P_2$ varies. (c) CTR of $P_1$ as $P_3$ varies. (d) CTR of $P_1$ as $P_4$ varies. (e) CTR of $P_1$ as $P_5$ varies.}
%     \label{fig:data_analysis}
% \end{figure*}

One of the challenges for page-level reranking is to model the intra- and inter-list interactions between items on a page. Therefore, we present a brief data-driven study on an F-shape page (i.e., Figure~\ref{fig:data_analysis_illustr}) to investigate how items at different positions influence each other. The data is collected from a mainstream App Store, where the page adopts an interleaved arrangement of vertical and horizontal lists. The detailed data description can be found in Section~\ref{sec:dataset}.

To study how the other items placed on the same page influence the utility of a given item, we select 6 fixed positions on the F-shape page, as illustrated in Figure~\ref{fig:data_analysis_illustr}. For the fixed position $P_1$:
\begin{itemize}[leftmargin=10pt]
    \item $P_2$ is adjacent to $P_1$ in the same list;
    \item $P_3$ is distant from $P_1$ in the same list;
    \item $P_4$ is adjacent to $P_1$ in another neighboring list;
    \item $P_5$ is distant from $P_1$ in another neighboring list;
    \item $P_6$ is distant from $P_1$ in a remote list.
\end{itemize}

They form five typical positional relationships on a multi-list page. For each pair of positions (i.e., $P_1$ versus $P_i$, $i=2,3,4,5,6$), we compute the click-through rate (CTR) of $P_1$ with different categories when the item category at $P_i$ varies. We plot the heatmap for the CTR w.r.t. the top five most frequent categories in Figure~\ref{fig:pos12} to \ref{fig:pos16}. Each symbol at the horizontal and vertical axes denotes an item category. The color variation represents how the CTR changes with the varying of the item category, and thereby reflects the items' mutual influences. From the figures, we have the following central observations (\textbf{Obs. I} to \textbf{Obs. III}):

% regarding the mutual influence between items on a multi-list page.
% \begin{enumerate}
%     \item Item utility is influenced by other items in the same list.
%     \item Item utility is influenced by other items across different lists.
%     \item The influence between items shows negative correlation with the distance between items.
% \end{enumerate}

\textbf{Obs. I:} \textit{Item utility is influenced by other items in the same list.} The greater the variation of the color in the heatmap, the stronger the influence between the items.  Figure~\ref{fig:pos12} ($P_2$) and~\ref{fig:pos13} ($P_3$) display how the CTR changes with the variation of the other items in the same list. 
It is evident that if the category of $P_1$ is fixed, the CTR of $P_1$ will vary with the category of $P_2$ and $P_3$. 
% Yet such influence between the two positions is asymmetric.
% Contrarily, the more uniform the color, the weaker the influence. 

% \xx{The two sentences seems irrelevant to observation I but more relevant to II and III}

\textbf{Obs. II:} \textit{Item utility is influenced by other items across different lists.} Figure~\ref{fig:pos14} to \ref{fig:pos16} show the inter-list interactions between items. 
% The CTR of $P_1$ in Figure~\ref{fig:pos14} to \ref{fig:pos16} varies with different categories in the other position, verifying the influence of items across different lists. 
The CTR of $P_1$ in Figure~\ref{fig:pos14} to \ref{fig:pos16} varies with different categories in the other position, verifying the item influence across lists. 
The color variation in the heatmap reflects the change in CTR, and further indicates the impacts of items. 
% In particular, although $P_4$ is placed in the different lists, its impact on $P_1$ is similar to $P_2$ (i.e., Figure~\ref{fig:pos12}) from the same list, which illustrates that inter-list interactions can be comparable to intra-list interactions for multi-list pages.
In particular, although $P_4$ (Figure~\ref{fig:pos14}) is placed in the different lists, its impact on $P_1$ is similar to $P_2$ (Figure~\ref{fig:pos12}) from the same list, illustrating that inter-list interactions can be comparable to intra-list interactions for multi-list pages.

\textbf{Obs. III:} \textit{The influence between items shows a negative correlation with the distance between items.} We adopt the Manhattan distance to measure the distance between two items to study how the distance affects the influence between them. The Manhattan distance is the sum of the difference on horizontal and vertical axes, as illustrated by the red auxiliary \emph{lines} and \emph{dots} in Figure~\ref{fig:data_analysis_illustr}. The distances from $P_1$ to $P_i\,(i=2,3,4,5,6)$ are $1$, $2$, $1$, $2$, $5$, respectively. Compared with Figure~\ref{fig:pos12}~($P_2$), the variation of the color in Figure~\ref{fig:pos13} ($P_3$) is more uniform, which suggests that the impact of a distant item is less than the adjacent ones in the same list. Similarly, for different lists, the CTR in Figure~\ref{fig:pos15} ($P_5$) and Figure~\ref{fig:pos16} ($P_6$) also varies more evenly than that in Figure~\ref{fig:pos14} ($P_4$). The light color of Figure~\ref{fig:pos16} is probably due to the fact that the dataset only records the observed data by the user, and the lower-ranked position $P_6$ is less observed with few data records when $P_1$ is clicked.


% % Comparing Figure~\ref{fig:pos13} with Figure~\ref{fig:pos12}, the variation of the color (CTR) is more uniform, which suggests that the impact of a distant item is less than the adjacent ones in the same list. 
% Compared with Figure~\ref{fig:pos12}~($P_2$), the variation of the color in Figure~\ref{fig:pos13} ($P_3$) is more uniform, which suggests that the impact of a distant item is less than the adjacent ones in the same list. 
% Similarly, for different lists, the CTR in Figure~\ref{fig:pos15} ($P_5$) and Figure~\ref{fig:pos16} ($P_6$) also varies more evenly than that in Figure~\ref{fig:pos14} ($P_4$). The light color of Figure~\ref{fig:pos16} is probably due to the fact that we only recorded exposure data.
% The backward position of $P_6$ has caused its fewer exposure data, probably mostly generated when the preceding item was not clicked, thus resulting in a lower CTR for $P_1$. 
% Therefore, we conclude that the more distant the items on the page, the less the mutual influence between them. 
% Moreover, there are various options for the distance measurement. For instance, in Figure~\ref{fig:data_analysis_illustr}, we adopt the Manhattan distance and illustrate the measurement by the red auxiliary \emph{lines} and \emph{dots}, which is the sum of the difference on horizontal and vertical axes. The distances from $P_1$ to $P_i\,(i=2,3,4,5,6)$ are $1$, $2$, $1$, $2$, $5$, respectively.

% \textbf{Observation 2:} There is cross-list interaction between the items on the page, and it is comparable to the intra-list interaction. Except for $P_1$ and $P_1$, all the three pairs of positions in Figure~\ref{fig:pos13}-\ref{fig:pos15} are cross-list position pairs, but the mutual influence between items is still apparent. Furthermore, the magnitude of the color change in the heatmap is an indicator of the magnitude of the change in CTR so as to reflect the magnitude of the mutual influence.  Figure~\ref{fig:pos13} presents a similar magnitude of color change to Figure~\ref{fig:pos13}, illustrating that the interaction between $P_1$ and $P_3$, not in the same list, can be comparable to the interaction between $P_1$ and $P_2$ in the same list.

% \textbf{Observation 3:} The more distant the items on the page, the weaker the interaction between them. The greater the color change in the heatmap, the stronger the influence between the items, and on the contrary, the more uniform the color, the weaker the influence. $P_1$ and $P_3$ lie in separate lists but adjacent to each other, so Figure~\ref{fig:pos13} shows a similar color change to Figure~\ref{fig:pos12}, where $P_1$ and $P_2$ are also adjacent. In figure~\ref{fig:pos14}, which shows the non-adjacent $P_1$ and $P_4$, the CTR varies evenly, implying that the interaction between $P_1$ and $P_4$ has diminished. As we move to $P_5$, which is more distant from $P_1$, the colors become more uniform in Figure~\ref{fig:pos15}, except for some outliers due to the small amount of data. This indicates that as the distance increases, the interaction between the two positions becomes weaker.

Therefore, we are motivated to propose a page-level reranking model that is aware of intra- and inter-list interactions and the spatial relationships between items across lists. 

\section{Methodology}


\begin{figure*}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.99\textwidth]{figures/frameworkv7.pdf}
    \vspace{-10pt}
    \caption{The overall framework of PAR, which consists of three major layers: (1) embedding layer, (2) page-level interaction layer, and (3) score estimation layer.}
    \vspace{-10pt}
    \label{fig:framework}
\end{figure*}
\subsection{Problem Formulation}

A page-level reranking model takes as inputs the multiple ordered initial lists on the same page generated by the previous rankers, and refines the ranking lists by considering the mutual influence between items and the impact of the page format.


For a user $u$ with the associated history list $H_u=[h_1^u,\ldots,h_t^u]$, and a multi-list page $P\in\mathcal{P}$ of $n$ different initial lists $\{R_1,R_2,\dots,R_n\}$, the problem of the page-level reranking is to jointly rerank the $n$ lists to optimize the overall utility by considering the page-wise context. 
Here, $t$ is the maximum length of the user's history list, $h_s^u$, $s=1\ldots,t$ is the $s$-th item recently clicked by the user $u$, $\mathcal P$ is the page set, and $R_i$, $i=1,\ldots,n$ is the $i$-th list with $m_i$ items. 
Let $m$ be the maximum length of the lists on the page. Then the whole page of candidate items to be reranked can be represented by an item matrix $\mathbf{X}_{n\times m}$, where $x_{i,j}$ denotes the $j$-th item in the $i$-th list, with all lists padded to the maximum length $m$. The utility of a page is defined by the expected sum (or weighted sum) of the click\footnote{The click could be replaced by other utility metrics like conversions, purchases, etc.} probability for each item on the page. 


% Given a set of users $\mathcal{U}=\{1,2,\ldots,N_u\}$ with the associated history list $H_u=[h_1^u,\ldots,h_t^u]$, a set of items $\mathcal{V}=\{1,2,\ldots,N_v\}$, and a multi-list page $\mathcal{P}=\{R_1,R_2,\dots,R_n\}$ of $n$ initial lists, the problem of the page-level reranking is to jointly rerank the $n$ lists to optimize the overall utility by considering the page-wise context. 
% Here, $N_u$ and $N_v$ denote by the number of users, and the number of items respectively, $t$ is the maximum length of the user's history list, and $R_i\in \Pi_{m_i}\left(\mathcal{V}\right)$, $i=1,\ldots,n$ is the $i$-th list with $m_i$ items. 
% Let $m$ be the maximum length of the lists on the page. Then the whole page of candidate items to be reranked can be represented by an item matrix $\mathbf{X}_{n\times m}$, where $x_{i,j}$ denotes the $j$-th item in the $i$-th list, with all lists padded to the maximum length $m$. The utility of a page is defined by the expected sum (or weighted sum) of the click probability\footnote{The click probability could be replaced by other utility metrics like conversions, purchases, etc.} for each item on the page. 

\label{sec:framework}


\vspace{-5pt}
\subsection{Model Overview}
We present Page-level Attentional Reranking (PAR) model and introduce how PAR captures the multifaceted fine-grained interactions for the whole page. As depicted in Figure~\ref{fig:framework}, PAR is an end-to-end reranking model, consisting of three layers: (1) embedding layer, (2) page-level interaction layer, and (3) score estimation layer.

\emph{Firstly}, the embedding layer converts each candidate or historical item to a dense feature vector. 
\emph{Then}, in the page-level interaction layer, we design three modules (i.e., hierarchical dual-side attention, spatial-scaled attention, and dense network) to capture page-wise information. 
% \emph{Then}, we design three modules (i.e., the hierarchical dual-side attention, spatial-scaled attention, and dense network) for the page-level interaction. 
% The hierarchical dual-side attention generates a shared page representation by extracting the intra- and inter-list interactions according to users' personalized behavior history.
% The spatial-scaled attention module captures the pairwise spatial relationship between item pairs with a designed distance matrix. The page format information is explicitly injected into the module.
% The dense network is shared for all the candidate items to facilitate implicit feature interactions.
\emph{Finally}, we adopt Multi-gated Mixture-of-Experts to learn the commonalities and distinctions among different lists and output the predicted score in the score estimation layer.
% we concatenate the extracted interaction features as the input for the reranking score estimation. 
\vspace{-8pt}
\subsection{Embedding Layer}

PAR applies the embedding layer to transform the sparse raw features into low-dimensional dense embedding vectors. The embedding layer takes as input both the candidate item matrix and the user's history list. Specifically, let $\hat{x}_{i,j}\in \mathbb R^{d_x}$ be the embedding of the item $x_{i,j}$, $i=1,\ldots,n$, $j=1,\ldots,m$ from the candidate item matrix, and $\hat h_s\in \mathbb R^{d_h}$ be the embedding of the item $h_s$, $s=1,\ldots,t$ from the history list, where $d_x$ and $d_h$ are the embedding size for the candidate and history items, respectively. 
We obtain the candidate item embedding matrix $\hat{\mathbf{X}}\in\mathbb{R}^{n\times m\times d_x}$ and the history item embedding matrix $\hat{\mathbf{H}}\in\mathbb{R}^{t\times d_h}$ after the embedding layer, where $t$ is the history length, $n$ is the number of lists, and $m$ is the number of items in each list.


\subsection{Page-level Interaction}

To fully exploit the page-wise information, we propose three modules in the page-level interaction layer: (i) The hierarchical dual-side attention (HDS-Attn) module learns the personalized intra- and inter-list interactions, and generates a shared page representation; (ii) The spatial-scaled attention (SS-Attn) module models the pairwise fine-grained item influence with the awareness of the page format effect; (iii) The dense network captures implicit feature interactions within each item. Detailed descriptions for each module are given in the following sections.

\subsubsection{Hierarchical Dual-side Attention}

One of the challenges of page-level reranking is to incorporate intra- and inter-list interactions on a page (\textbf{C1} in Section~\ref{sec:intro}). Since there is a natural hierarchical structure of \emph{items forming a list} and \emph{lists forming a page}, we propose to consider intra-list and inter-list interaction in a hierarchical way. As shown in the left part of Figure~\ref{fig:framework}, the HDS-Attn module consists of dual-side attention, item-level aggregation, list-level self-attention, and list-level aggregation, from bottom to top. The bottom two parts are designed to extract the intra-list interaction within each list. To provide personalized reranking, the cross-item influence on the candidate item side requires the personal preference information from the history list side. Therefore, we introduce the dual-side attention for each list to model the mutual influence between these two sides. Then, item-level aggregation is employed to combine the item information within a list and generate \textit{list representation}. The upper two parts, list-level self-attention and list-level aggregation, are designed to capture the inter-list interaction between different lists and generate the final \textit{page representation}. 
% We propose the hierarchical dual-side attention (HDS-Attn) to enable the automatic learning of the personalized intra- and inter-list interactions at various levels. 
% As shown in the left part of Figure~\ref{fig:framework}, the hierarchical structure synchronously extracts four different levels of interactions including dual-side attention, item-level aggregation, list-level self-attention, and list-level aggregation, from bottom to top.

% First, users' history behaviors can reflect their personalized preferences, thus affect the reranking of the candidate items. Therefore, we introduce the dual-side attention for each list to model the mutual influence between the two sides, history list and candidate items. 

\smallskip
\noindent \textbf{Dual-side Attention.} Users' history list carries rich information for inferring their personal preferences and tastes, which is helpful for reranking~\cite{xi2022multi,li2022pear}. Moreover, the items in the users' history list contribute differently for different candidate lists~\cite{xi2022multi,qin2020user}. For example, game apps in the user's history list may be more important when reranking the "Top-10 Games" list for the user. Inspired by~\cite{co_att}, we design the dual-side attention to model the fine-grained correlations between the candidate item side and history list side.


Formally, for each list $R_i$ on page $P$, $i=1,\ldots,n$, the input of the dual-side attention is the corresponding $i$-th embedding matrix $\hat{\mathbf{X}}_i\in\mathbb{R}^{m\times d_x}$ of the candidate list and the history embedding matrix $\hat{\mathbf{H}}\in\mathbb{R}^{t\times d_h}$.
We maintain an affinity matrix $\mathbf{W_a}\in\mathbb{R}^{d_h \times d_x}$ to learn the importance of the association between each pair of items from both candidate and history sides:
\begin{equation}
\begin{split}
    \mathbf{C}_i&=\tanh{(\hat{\mathbf{H}}\mathbf{W}_{a}\hat{\mathbf{X}}_i^\top )}\,, \\
    \mathbf{A}_i^x&=\operatorname{Softmax}\left(\tanh{(\hat{\mathbf{X}}_i\mathbf{W}_x+(\hat{\mathbf{H}}\mathbf{W}_h)^\top \mathbf{C}_i)}\right),\\
    \mathbf{A}_i^h&=\operatorname{Softmax}\left(\left(\tanh{(\hat{\mathbf{H}}\mathbf{W}_h + \mathbf{C}_i(\hat{\mathbf{X}}_i\mathbf{W}_x))}\right)^\top\right),\\
    \Tilde{\mathbf{X}}_i&=\mathbf{A}_i^x\hat{\mathbf{X}}_i\,,\;\;\;\;\;\Tilde{\mathbf{H}}_i=\mathbf{A}_i^h \hat{\mathbf{H}}\,,
\end{split}
\label{eq:dual-side attention}
\end{equation}
where $\mathbf{W}_x\in\mathbb{R}^{d_x\times m}, \mathbf{W}_h\in\mathbb{R}^{d_h\times m}$ are learnable weight matrices. 
The matrices $\mathbf{A}_i^x\in\mathbb{R}^{m\times m}$ and $\mathbf{A}_i^h\in\mathbb{R}^{t \times m}$ after the softmax function represent the attention weights of items in the candidate list and history list. 
Then the interacted representation matrices $\Tilde{\mathbf{X}}_i=[\Tilde{\mathbf{x}}_{i,j}]_{j=1}^m\in\mathbb{R}^{m\times d_x}$ and $\Tilde{\mathbf{H}}_i=[\Tilde{\mathbf{h}}_{i,j}]_{j=1}^m\in\mathbb{R}^{m\times d_h}$ now contain useful information from both candidate list $R_i$ and history list $H_u$. 

\smallskip
\noindent \textbf{Item-level Aggregation.}
We apply the item-level aggregation to learn the intra-list interaction, and generate the list representations.
Since items contribute differently to the representation of the target list $R_i$, we aggregate the attained item representations with an attention mechanism \cite{yang-etal-2016-hierarchical} to form the \textit{list representation} $l_i$:
\begin{equation}
\begin{split}
    u_{i,j} &= \tanh{(\mathbf{W}_l[\Tilde{\mathbf{x}}_{i,j} \,\Vert\, \Tilde{\mathbf{h}}_{i,j}] + b_l)}\,,\\
    \alpha_{i,j}& =\frac{\text{exp}(u_{i,j}^\top  q_{\text{item}})}{\sum_{j'=1}^{m} \text{exp}(u_{i,j'}^\top q_{\text{item}})}\,,\\
    % \alpha_{i,j}& =\operatorname{Softmax}_k(u_{i,k}^\top  q_{\text{item}}),\,j=1,\dots,m,\\
    l_i& =\sum\nolimits_{j=1}^m{\alpha_{i,j}[\Tilde{\mathbf{x}}_{i,j} \,\Vert\, \Tilde{\mathbf{h}}_{i,j}]}\,,\\
\end{split}
\end{equation}
where $\Vert$ denotes the vector concatenation.
We first feed the concatenated item representations into a linear layer to get $u_{i,j}$ for each item $x_{i,j}$, where $\mathbf{W}_l\in\mathbb R^{d_l\times d_l}$ and $b_l\in\mathbb R^{d_l}$ ($d_l=d_x+d_h$) are the learnable weights. Then the importance of each item is measured by the similarity of $u_{i,j}$ with a item-level query vector $q_{\text{item}}\in\mathbb{R}^{d_l}$. The item-level query vector $q_{\text{item}}$ is a trainable parameter and serves as the attention query in the item-level aggregation. Next, we normalize the weights $\alpha_{i,j}$ and compute the list representation $l_i$ by the weighted sum of each item. To this end, important intra-list interaction has been fused into the list representation $l_i$. Stacking all the list representations, we get the list representation matrix $\textbf{L}=[l_i]_{i=1}^n\in\mathbb{R}^{n\times d_l}$ for further use. 

\smallskip
\noindent \textbf{List-level Self-attention.}
Given the list representation matrix $\textbf{L}$, we model the inter-list influence between different lists on the page through a list-level self-attention layer:
\begin{equation}
    \Tilde{\mathbf{L}}=\text{Softmax}\left(\frac{\mathbf{L}\mathbf{L}^\top}{\sqrt{d_l}}\right)\mathbf{L}\,,
\end{equation}
where $\Tilde{\mathbf{L}}=[\Tilde{l}_i]_{i=1}^n \in \mathbb R^{n\times d_l}$ is the re-weighted list representation matrix that captures the relationship and correlations between different lists, and $\sqrt{d_l}$ is used to stabilize gradients during training.

  
\smallskip
\noindent \textbf{List-level Aggregation.}
Finally, built upon the re-weighted list representations $\Tilde{\mathbf{L}}$, we employ the list-level aggregation layer to combine the information from different lists and generate the unified page representation $S$. Similar to the item-level aggregation, after a linear transformation,  we involve a learnable list-level query vector $q_{\text{list}}\in\mathbb{R}^{d_l}$ for calculating the attention weights $\beta$. Then the re-weighted list representations $\Tilde{\textbf{L}}$ are aggregated into a shared \textit{page representation} $S$ by a weighted sum:
\begin{equation}
\begin{split}
    v_i& = \tanh{(W_p \Tilde{l}_i + b_p)}\,,\\
    % \beta_i& =\operatorname{Softmax}_i(v_i^\top q_{\text{list}}),\;i=1,\dots,n,\\
    \beta_i& =\frac{\text{exp}(v_i^\top q_{\text{list}})}{\sum_{i'=1}^n \text{exp}(v_{i'}^\top q_{\text{list}})}\,,\\
    S& =\sum\nolimits_{i=1}^n{\beta_i \Tilde{l}_i}\,,\\
\end{split}
\end{equation}
where page representation $S$ integrates the information of page-wise contexts and history behaviors, and is shared for all the lists.


\subsubsection{Spatial-scaled Attention}
\label{sec:spatial-scaled attention}
With multiple lists on one page, the arrangement of lists and items, i.e., the page format, becomes an essential issue to be considered (\textbf{C2} in Section~\ref{sec:intro}). 
However, no previous work on page-level reranking has discussed such an issue before. Different page formats change the location of items and therefore change the distances between them. In Section~\ref{sect:data_analysis}, we observe that the mutual influence between items generally shows a negative correlation with the distance between them. Hence different page formats yield diverse mutual influences between items. 
Thus, we propose the SS-Attn module to estimate the pairwise item influence with the consideration of the spatial relationship. Specifically, SS-Attn adjusts the attention weights according to the relative distance between items on the page, so that closer items have a stronger influence on each other. The relative distance can be altered depending on the page format, showing that the SS-Attn is flexible and can be adapted to different formats.

% Furthermore, to keep the precise spatial relationship between items across lists, we propose the spatial-scaled attention (SS-Attn) module. SS-Attn estimates the pairwise item influence by considering the page format information -- the spatial layout and the distance between items. As discussed in Section~\ref{sect:data_analysis}, the mutual influence between items generally shows negative correlation with the distance between items, which directly reflects the page format effect. 

As such, with a total of $nm$ items on the page, we introduce a symmetric distance matrix $\mathbf{D}\in\mathbb{R}^{nm \times nm}$, whose element $d_{p, q}\ge 0$ indicates the geometric distance between the corresponding pair of items $(p, q)$. In this work, we adopt the Manhattan distance to build the distance matrix. 
For example, in Figure~\ref{fig:data_analysis_illustr}, the Manhattan distances from $P_1$ to $P_i\,(i=2,3,4,5,6)$ are $1$, $2$, $1$, $2$, $5$, respectively.
It is worth noting that the design of the distance matrix is flexible and can be customized according to the page formats in different page-level reranking scenarios. Other distance measurements (e.g., Euclidean distance, slot counting) are also applicable.


Concretely, we first reshape the embedding matrix of the candidate items $\hat{\mathbf{X}}\in \mathbb{R}^{n\times m \times d_x}$ into $\Bar{\mathbf{X}}\in \mathbb{R}^{nm\times d_x}$, where each row $\Bar{x}_{p}\,(p=1,\dots,nm)$ of the matrix $\Bar{\mathbf{X}}$ is the feature vector of a candidate item. The input of the SS-Attn module is the reshaped item matrix $\Bar{\mathbf{X}}$ and the distance matrix $\mathbf{D}$. 
To involve the page format effect (i.e., the larger the distance, the less the influence between items), we transform the distance matrix by a learnable sigmoid function~\cite{wu2021transformer}. 
% For item pair $(p,q)$, the learnable sigmoid function $f$ parameterized by a scalar $v$ is used to map the distance $d_{p,q}$ to a positive distance-aware influence factor $\hat{d}_{p,q}$ of range $(0,1]$, $f(\cdot|v):\mathbb N\rightarrow \mathbb (0,1]$.
The learnable sigmoid function $f$ parameterized by a scalar $v$ maps the distance $d_{p,q}$ of item pair $(p,q)$ to a positive distance-aware influence factor $\hat{d}_{p,q}$ of range $(0,1]$, $f(\cdot|v):\mathbb N\rightarrow \mathbb (0,1]$.
\begin{equation}
    \hat{d}_{p,q}=f(d_{p,q}|v)=\frac{1+\exp(v)}{1+\exp(v + \sigma d_{p,q})}\,,
\end{equation}
where $v\in\mathbb R$ is a learnable scalar that determines the steepness of function $f(\cdot|v)$, and $\sigma > 0$ is a hyper-parameter for normalizing the distance $d_{p,q}$ and stabilizing the training. In our experiment, $\sigma$ is set to $0.1$.  Note that $f(\cdot|v)$ is a monotonically decreasing function w.r.t. the distance and satisfies $f(0|v)=1$ and $f(+\infty|v)\rightarrow 0$, i.e., the influence of between the items gradually decreases from $1$ to $0$ as the distance grows.

Next, we use the obtained influence factor $\hat{d}_{p,q}$ to scale the pairwise mutual influence between items on the page. Multi-head attention is adopted for modeling the interactions between any pair of items on the page, while the attention weights are scaled according to the distance-aware influence factor. Suppose $B$ is the number of heads, we maintain $B$ different learnable sigmoid functions to learn different levels of the page format effect, with an individual parameter $v^{(b)}$ for the $b$-th attention head, $b=1,\ldots,B$. We form all the $\hat{d}_{p,q}$ for the $b$-th head into a matrix $\hat{\mathbf{D}}^{(b)}$, and numerically scale the preliminary self-attention weights:
\begin{equation*}
\begin{split}
    \Bar{\mathbf{O}}^{(b)}&=\operatorname{Softmax}\left(\frac{\phi((\Bar{\mathbf{X}}W_Q^{(b)})(\Bar{\mathbf{X}}W_K^{(b)})^\top)\odot \hat{\mathbf{D}}^{(b)}}{\sqrt{d_a}}\right)(\Bar{\mathbf{X}}W_V^{(b)}),
\end{split}
\end{equation*}
where $\odot$ is the element-wise product, the preliminary attention weights $(\Bar{\mathbf{X}}W_Q^{(b)})(\Bar{\mathbf{X}}W_K^{(b)})^\top$ are adjusted according to the distance-aware influence factors, and $d_a$ is the dimension of the vectors in $\Bar{\mathbf{X}}W_Q^{(b)}$
and $\Bar{\mathbf{X}}W_K^{(b)}$. Note that the non-negative monotonically increasing function $\phi$ is introduced to avoid negative attention weights, as negative preliminary attention weights can invert the distance-aware influence and violates the negative correlation between distances and influences. Here, we use $\operatorname{softplus}$ function.

% \operatorname{ReLU}

Finally, we concatenate the multi-head spatial-scaled attention outputs, and apply a linear transformation to get the pairwise influence matrix $\Bar{\mathbf{O}}\in\mathbb{R}^{nm\times d_o}$, $\Bar{\mathbf{O}} = [\Bar{\mathbf{O}}^{(1)}\,\Vert\,\dots\,\Vert\,\Bar{\mathbf{O}}^{(B)}]\mathbf{W}_O$,
% \begin{equation}
% \begin{split}
%     % \Bar{\mathbf{O}} &= \left[\Bar{\mathbf{O}}^{(1)}\,\Vert\,\dots\,\Vert\,\Bar{\mathbf{O}}^{(B)}\right]\mathbf{W}_O,
%     \Bar{\mathbf{O}} &= [\Bar{\mathbf{O}}^{(1)}\,\Vert\,\dots\,\Vert\,\Bar{\mathbf{O}}^{(B)}]\mathbf{W}_O,
% \end{split}
% \end{equation}
where $d_o$ is the attention output size. We reshape the matrix $\Bar{\mathcal{O}}\in\mathbb{R}^{nm \times d_o}$ back to $\mathbf{O}\in\mathbb{R}^{n \times m \times d_o}$, where the vector $o_{i,j} \in \mathbb{R}^{d_o}$ denotes the pairwise influence vector for the $j$-th item in the $i$-th list.



\subsubsection{Dense Network}

In addition to the HDS-Attn and SS-Attn, we employ a fully-connected network to capture the implicit feature interactions within each item. We feed each item embedding $\hat{x}_{i,j}$ into a shared MLP to obtain the dense feature $r_{i,j}=\operatorname{MLP}(\hat{x}_{i,j})$ for the latter reranking score estimation.
% \begin{equation}
%     r_{i,j}=\operatorname{MLP}(\hat{x}_{i,j}).
% \end{equation}

\subsection{Reranking Score Estimation}
% For the user $u$ and an initial page $\mathcal{P}$, the reranking score estimation computes the reranking score $\hat{y}_{i,j}$ for each candidate item $x_{i,j}$. 
The reranking score estimation computes the reranking score $\hat{y}_{i,j}$ for each candidate item $x_{i,j}$. 
After the page-level interaction layer, we obtain the shared page representation $S$, the pairwise item influence vector $o_{i,j}$, and the dense feature $r_{i,j}$ for each candidate item $x_{i,j}$. Although these features incorporate page-level and item-level information, the commonalities and distinctions of user behaviors on different lists are remained to be solved.


As discussed before (\textbf{C3} in Section~\ref{sec:intro}), the user's behaviors may not only share some basic patterns (e.g., position bias) and underlying preferences, but also have distinctions for different lists due to themes and formats. To this end, we adopt the Multi-gated Mixture-of-Experts (MMoE~\cite{ma2018modeling}) module, where several expert sub-models are shared across all lists. Each list possesses a specific gating network to "select" a subset of experts to
use. Through the expert and gating networks, our model automatically adjusts parameterization between modeling shared information and list-specific information, so as to exploit the common behavior patterns while paying attention to the list-specific patterns.

As shown in Figure~\ref{fig:framework}, there are $E$ parallel expert networks $\{e_k(\cdot)\}_{k=1}^{E}$, which are all MLPs with ReLU activations, to capture different aspects of behavior patterns. For each list $i$, we maintain a separate fully-connected gating network $g_i(\cdot)$ to learn a linear combination of the expert outputs. 
To preserve the list-specific information, we feed the combined feature vector $\hat{z}_{i,j}$ into a list-specific tower network $t_i(\cdot)$ to get the final reranking score $\hat{y}_{i,j}$ for the $j$-th item in the $i$-th list.
% \begin{equation}
% \begin{split}
%     z_{i,j} &= [S \,\Vert\, r_{i,j} \,\Vert\, o_{i,j}]\,,\\
%     \gamma_{i,j,k} &=\operatorname{Softmax}_k(g_i(z_{i,j})),\;k=1,\dots,E\,,\\
%     \hat{z}_{i,j}&=\sum\nolimits_{k=1}^{E} \gamma_{i,j,k} \times e_k(z_{i,j})\,,\\
%     \hat{y}_{i,j} &= t_i(\hat{z}_{i,j})\,. \\
% \end{split}
% \end{equation}
\begin{equation}
\begin{split}
    % z_{i,j} &= [S \,\Vert\, r_{i,j} \,\Vert\, o_{i,j}]\,,\\
    \gamma_{i,j,k} &=\operatorname{Softmax}_k(g_i([S \,\Vert\, r_{i,j} \,\Vert\, o_{i,j}])),\;k=1,\dots,E\,,\\
    \hat{z}_{i,j}&=\sum\nolimits_{k=1}^{E} \gamma_{i,j,k} \times e_k([S \,\Vert\, r_{i,j} \,\Vert\, o_{i,j}])\,,\\
    \hat{y}_{i,j} &= t_i(\hat{z}_{i,j})\,. \\
\end{split}
\end{equation}

% The final rerankings can be achieved by sorting the items in each list $i$ according to the estimated scores $\hat{y}_{i,j},\,j=1,\dots,m$.
We sort items in each list by the scores $\hat{y}_{i,j}$ to get the final rerankings.
Given the click label matrix $\mathbf{Y}$ of size $n\times m$ where $y_{i,j}$ denotes the click signal for the $j$-th item in the $i$-th list, we optimize the model via binary cross-entropy loss on the training page set $\mathcal P$:
% \begin{equation}
%     \mathcal{L}=\sum_{u \in \mathcal{U}}\sum_{\mathcal{P}\in \mathcal{P}_u}\sum_{i=1}^n\sum_{j=1}^m y_{i,j}\log \hat{y}_{i,j} + (1-y_{i,j})\log(1-\hat{y}_{i,j})\,.
% \end{equation}
\begin{equation}
    \mathcal{L}=\sum_{\mathcal{P}}\sum_{i=1}^n\sum_{j=1}^m y_{i,j}\log \hat{y}_{i,j} + (1-y_{i,j})\log(1-\hat{y}_{i,j})\,.
\end{equation}
% where $\mathcal T$ is the training dataset contains all the training pages.
% \subsection{Computational Complexity Analysis}
% \textbf{Computational Complexity Analysis.} The complexity of PAR is $\mathcal O(n^2m^2)$, where $n$ is the number of lists, $m$ is the length of the lists. Its complexity is comparable to most existing models of  $\mathcal O(nm^2)$ (e.g., PRM~\cite{pei2019personalized}, DHANR~\cite{ding2019whole}), as the number of lists on the page $n$ is usually less than 5 due to the limit of the screen size. 
% The computation of the page-level interaction can be made parallel to further accelerate the process.  


% For the traditional practice that uses $n$ individual list-level reranking models (e.g., PRM~\cite{pei2019personalized}, SetRank~\cite{pang2020setrank}) for each of the $n$ lists, the complexity is $\mathcal O(nm^2)$, where $m$ is the maximum length of the list. While for PAR, the complexity is $\mathcal O(n^2m^2)$. The additional complexity cost is brought by computing the page-level interactions. However, the number of lists on the page $n$ is usually less than 5 due to the limit of the screen size. Therefore, the cost is inexpensive for PAR. Moreover, the computation of the page-level interaction can be made parallel to further accelerate the process.  

\section{Experiment}
\label{sec:exp}
% In this section, we first compare our proposed PAR with the state-of-the-art baselines. Then, we investigate the impact of several critical components of PAR, followed by a case study to explore how PAR captures the inter-list interactions and the spatial relationship between items.
\subsection{Experiment Settings}
\subsubsection{Datasets}\label{sec:dataset} To study the effectiveness of PAR, we conduct experiments on a public dataset, Cloud Theme Click Dataset\footnote{https://tianchi.aliyun.com/dataset/dataDetail?dataId=9716}, and a proprietary dataset, AppStore.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{Cloud Theme Click Dataset}~\cite{du2019sequential} (\textbf{CTC} for short) records the click data of Cloud Theme in Taobao App. The dataset includes 1,423,835 click records from 355 different themes during a 6-day promotion season, users'  purchase history before the promotion, and the embedding of 720,210 users and 1,361,672 items. 
    % The dataset includes 1,423,835 clicks records from 355 different themes during a 6-day promotion season, users'  one-month purchase history before the promotion, the item pool of each theme, and the 128-dimension embedding of 720,210 users and 1,361,672 items. 
    \item \textbf{AppStore} is collected from a mainstream commercial app store, from October 16, 2021 to November 1, 2021. The dataset contains 47,003,121 pages, 28,632,998 users and 1365 apps. Each app has 32 features (e.g., app developer, app category). Each page is in the form of an F-shape with one vertical list inserted by four horizontal lists, and each user has a history list of behaviors collected in real time.
    % \item \textbf{AppStore} is collected from a mainstream commercial app store, from October 16, 2021 to November 1, 2021.  The dataset contains 394,046 queries and 1646 apps. Each app has 32 features (e.g., app developer, app category). Each page is in the form of an F-shape with one vertical list inserted by four horizontal lists, and each user has a history list of behaviors collected in real time.
\end{itemize}
\vspace{-5pt}
\subsubsection{Page and click generation for public dataset}\label{page_click} As there is \textbf{no publicly available} dataset with page data, we use the click logs of the public CTC dataset to construct the pages. For each user, we first construct lists from her/his positively interacted themes with at least one click. Next, each page is formed by four lists from different themes that are horizontally stacked from top to bottom. We randomly sample lists from all the themes if less than four lists have been clicked. Four DNN models are trained separately as the initial rankers to generate the initial rankings of length 10. 

% Each page has four lists from different themes that are horizontally stacked from top to bottom. For each user, input pages are constructed from positively interacted lists with at least one click. We randomly sample lists from all the themes if less than four lists have been clicked by the user. The length of the initial list is 10. Four DNN models are trained separately as the initial ranker to generate the initial rankings. 

An oracle click model is then adopted to simulate necessary click data on the obtained new pages. We mainly follow the click simulation in Seq2Slate \cite{bello2018seq2slate} to decompose the click probability of an item into the product of relevance, position decaying, and dissimilarity probability. We use the original click label of an item as the relevance probability, which is equal to $1$ if clicked, and $0$ otherwise. If the item is placed at $i$-th position in the $j$-th list, the position decaying probability is $1/(i^{\eta_1}j^{\eta_2})$, where $\eta_1$ and $\eta_2$ are the horizontal and vertical decay parameters. Here we set $\eta_1$ and $\eta_2$ to 0.4 and 0.5. When observing an item, the user may tend to click the item dissimilar/diverse to its surrounding items~\cite{diverOrNot, clkToDiver}. The cosine similarity between item embeddings is used to compute the dissimilarity probability to introduce high-order interaction between items. After the generation of clicks, all baselines and our model PAR are trained based on the synthetic click data.
\vspace{-5pt}
\subsubsection{Baselines} 
% We compare our proposed PAR with the state-of-the-art page-level baselines, including page-level reranking model \textbf{DHANR}, multi-scenario LTR model \textbf{HMoE} and whole-page optimization work \textbf{TRNN}.
Since currently there is only one work, \textbf{DHANR}, that focuses on page-level reranking, we modify some models in related fields that utilize page-level information as baselines, e.g.,  \textbf{HMoE} in multi-scenario ranking, \textbf{TRNN} in whole-page optimization. We also design \textbf{GlobAtt} to directly model the influences between items on a page. The relationship and differentiation between page-level reranking and the related fields are discussed in Section~\ref{sect:related}.
\begin{itemize}[leftmargin=10pt]
    % \item \textbf{DHANR}~\cite{hao2021re} applies a hierarchical attention network to progressively aggregate the item features into a unified page representation. The obtained page representation is used as shared side information to help the list-level reranking in each list.
    \item \textbf{DHANR}~\cite{hao2021re} applies a hierarchical attention network to aggregate the item features into a unified static page representation, which is shared for the list-level reranking in each list.
    % \item \textbf{HMoE}~\cite{li2020improving} takes advantage of Multi-task Mixture-of-Experts to implicitly identify distinctions and commonalities between lists from different scenarios in the feature space.
    \item \textbf{HMoE}~\cite{li2020improving} adopts MMoE to implicitly identify distinctions and commonalities among lists from different scenarios.
    \item \textbf{TRNN}~\cite{lo2021page} focuses on whole-page optimization and ranks the widgets (fixed ordered lists) by a two-stage RNN. Necessary modifications to TRNN are made so that it can employ the page information to help rerank the items in different lists.
    \item \textbf{GlobAtt} fuses multiple lists into one mixed list and adopts a global multi-head self-attention structure to model the mutual influence between any pairs of items on the page. List and position context are fed into the network as additional features.
\end{itemize}

We also deploy list-level reranking for multiple lists on the same page. Multiple models are trained separately on different lists.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{miDNN}~\cite{zhuang2018globally} uses global feature extension to extract mutual influence between items in each ranking list.
    \item \textbf{GSF}~\cite{ai2019learning} employs deep neural networks (DNN) to learn multivariate scoring functions by enumerating feasible item permutations.
    \item \textbf{DLCM}~\cite{ai2018learning} applies gated recurrent units (GRU) to encode top items in the ranking lists into feature representations.
    \item \textbf{PRM}~\cite{pei2019personalized} models the mutual influence between any pairs of items and users' preferences by self-attention.
    \item \textbf{SetRank}~\cite{pang2020setrank} learns permutation-equivariant representations for the inputted documents via the self-attention structure.
\end{itemize}


\begin{table*}[]
    \vspace{-10pt}
    \caption{Overall performance on the AppStore and CTC datasets.}
    \label{tab:overall}
    \vspace{-10pt}
    \centering
\setlength{\tabcolsep}{2pt}
% \scalebox{0.79}{
\begin{adjustbox}{max width=0.925\linewidth}
    \begin{tabular}{c|ccccccccc|cccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{9}{c}{\textbf{AppStore dataset}}  & \multicolumn{8}{c}{\textbf{CTC dataset}}  \\
    \cmidrule{2-18}
    & $\mathbf{Utility}$            & $\mathbf{CTR}$             & $\mathbf{CTR_v}$          & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{CTR_{h4}}$         & $\mathbf{nDCG}$            & $\mathbf{MAP}$             & $\mathbf{Utility}$            & $\mathbf{CTR}$             & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{nDCG}$             & $\mathbf{MAP}$              \\
    \midrule
    INIT                             & 1.0459           & 1.0571           & 0.2896           & 0.6953           & 0.0391          & 0.0122          & 0.0098          & 0.6260          & 0.5087          & 1.2706           & 1.2545           & 0.5030           & 0.3747           & 0.3161          & 0.0607          & 0.4953           & 0.3241           \\
    miDNN                            & 1.1704           & 1.1993           & 0.3428           & 0.7588           & 0.0396          & \textbf{0.0186} & 0.0107          & 0.6375          & 0.5204          & 1.3530           & 1.3305           & 0.5302           & 0.3884           & 0.3439          & 0.0680          & 0.5090           & 0.3415           \\
    GSF                              & 1.2183           & 1.1866           & 0.3970           & 0.7505           & 0.0420          & 0.0146          & 0.0142          & 0.6344          & 0.5171          & 1.2791           & 1.3252           & 0.5308           & 0.3899           & 0.3386          & 0.0659          & 0.5238           & 0.3618           \\
    DLCM                             & 1.3218           & 1.2593           & 0.4521           & 0.8052           & 0.0361          & 0.0176          & 0.0107          & 0.6234          & 0.5020          & 1.3494           & 1.3603           & 0.5371           & 0.4064           & 0.3504          & 0.0664          & 0.5303           & 0.3692           \\
    PRM                              & 1.3438           & 1.2748           & 0.4497           & 0.8242           & 0.0430          & 0.0151          & 0.0117          & \textbf{0.6403}          & \textbf{0.5238} & 1.3722           & 1.3710           & 0.5474           & 0.4014           & 0.3539          & 0.0684          & 0.5212           & 0.3578           \\
    SetRank                          & 1.3535           & 1.2938           & 0.4863           & 0.8013           & 0.0366          & 0.0166          & 0.0127          & 0.6388   & 0.5223          & 1.3643           & 1.3635           & 0.5432           & 0.4026           & 0.3507          & 0.0671          & 0.5300           & 0.3689           \\ \midrule
    GlobAtt	& 1.3896 & 1.3611 & 0.5335 &	0.7586 &	0.0415 &	0.0169 &	0.0107 & 0.6245 &	0.5033 &	1.3678 &	1.3638 &	0.5449 & 	0.4039 &	0.3474 & 	0.0676 &	0.5185  & 0.3538\\
    TRNN                             & 1.3970           & 1.3641           & 0.5029           & 0.7899           & 0.0431          & 0.0172          & 0.0111          & 0.6351          & 0.5172          & 1.3750           & 1.3602           & 0.5533           & 0.3965           & 0.3430          & 0.0674          & 0.5220           & 0.3587           \\
    HMoE                             & 1.3706           & 1.3744           & 0.5394           & 0.7661           & 0.0414          & 0.0167          & 0.0108          & 0.6373          & 0.5203          & 1.3615           & 1.3608           & 0.5452           & 0.3968           & 0.3492          & \textbf{0.0696} & 0.5236           & 0.3609           \\
    DNAHR                            & 1.4116           & 1.3872           & 0.5312           & 0.8213           & 0.0405          & 0.0107          & 0.0078          & 0.6312          & 0.5121          & 1.3303           & 1.3512           & 0.5382           & 0.3992           & 0.3450          & 0.0687          & 0.5233           & 0.3597           \\
    \textbf{PAR}                     & \textbf{1.5024*} & \textbf{1.4457*} & \textbf{0.5801*} & \textbf{0.8413*} & \textbf{0.0503} & 0.0161          & \textbf{0.0146} & 0.6333          & 0.5151          & \textbf{1.4446*} &	\textbf{1.4137*} &	\textbf{0.5693*} &	\textbf{0.4174*} &	\textbf{0.3594} &	0.0677	 & \textbf{0.5548*} &	\textbf{0.4005*}\\
    \bottomrule
    \end{tabular}
\end{adjustbox}
% }
\footnotesize \flushleft\hspace{0.6cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
\vspace{-10pt}
\end{table*}


\subsubsection{Evaluation metrics} All the reranking models are evaluated in terms of relevance-based and utility-based metrics. For relevance-based metrics, we adopt widely-used \textit{MAP} and \textit{nDCG}~\cite{ndcg} following previous work \cite{lo2021page,pei2019personalized, ai2018learning}. Despite that there are multiple lists on the page, we calculate \textit{nDCG} and \textit{MAP} for each list and report their averaged \textit{nDCG} and \textit{MAP}.


As for utility-based metrics, we employ the average number of clicks on the page \textit{Utility}, and the click probability per page (i.e., the sum of item click probability on a page) \textit{CTR}, following~\cite{xi2021context}. In addition, we also compute the average click probability on each list, such as the average click probability on vertical lists $CTR_v$, and the average click probability on the first horizontal lists $CTR_{h1}$. The click probabilities and clicks on the public CTC dataset are generated by the same oracle click model used in \ref{page_click}. The AppStore dataset records the real user clicks on the F-shape page for evaluation of \textit{Utility}, while the click probabilities are given by an oracle click model for the F-shape page, FSCM~\cite{fu2022f}.

\subsubsection{Reproducibility}
The implementation of our model is publicly available\footnote{Our code is available at https://anonymous.4open.science/r/PAR-CDCE}. We adopt Adam as the optimizer. The learning rate is 
$2\times10^{-4}$, and the parameter of $l_2$ regularization is $2\times 10^{-4}$. The batch size and the embedding size of the categorical feature are set to 128 and 16. The number of experts and the architecture of experts and towers in MMoE are 12, [200, 80], and [80], respectively. To ensure a fair comparison, we also fine-tune all  baseline models to achieve their best performance. 

% On the CTC dataset, there are four horizontal lists on the page with each list having a length of 10, and the maximum length of user behavior sequences for each user is 10. 
%  The number of experts and the architecture of experts and towers in MMoE are 12, [200, 80], and [80], respectively. 

\subsection{Overall Performance}
The overall performance of our proposed PAR and baselines on the AppStore and CTC datasets are reported in Table \ref{tab:overall}, from which we have the following observations.

\textit{ Firstly, our model PAR performs significantly better than all the baselines on both datasets.} Methods with page-wise information such as HMoE, TRNN, DHANR, and GlobAtt generally work better than list-level methods, validating the benefit of utilizing page-level information. PAR surpasses all the baselines on the two datasets. As presented in Table~\ref{tab:overall}, PAR improves over the best baseline on CTC dataset with respect to \textit{Utility}, \textit{CTR}, \textit{nDCG}, and \textit{MAP} by 5.276\%, 3.115\%, 4.623\%, and 8.485\%, respectively. On AppStore dataset, PAR also achieves 6.432\% and 4.217\% improvement over the best baseline in terms of \textit{Utility} and \textit{CTR}.
This demonstrates the necessity of modeling the multifaceted dynamic interactions and the page format  in page-level reranking. 
% This demonstrates the necessity of modeling the page format and the relationship between different lists in page-level reranking. PAR is aware of the multifaceted dynamic interactions as well as the page format of the whole page.

\textit{Secondly, different page formats result in different click distributions. }As illustrated in Table~\ref{tab:overall}, the top clicks are predominantly located on the vertical and the first horizontal lists on the F-shape pages of AppStore dataset. On the all-row pages of CTC dataset, clicks are concentrated on the first three horizontal lists and the probability of clicking decreases with the positions of the horizontal list. PAR shows greater improvement in these major lists by exploiting more useful information. Page-level baselines outperform list-level models on AppStore dataset, but sometimes this is not the case for the CTC dataset, which may also be due to the different page formats. The inter-list interaction for pages of multiple horizontal lists may be less than that for F-shape pages.

\textit{Lastly, the performance of the models on the AppStore and CTC datasets diverges in terms of the relevance-based metrics, \textit{nDCG} and \textit{MAP}.} On the CTC dataset, PAR achieves the best nDCG and MAP, but on the AppStore dataset, the best relevance-based metrics are achieved by the list-level reranking method, PRM. 
% This may be because of the labels given in the datasets. 
This may be attributed to the fact that CTC dataset has groundtrue relevance labels, whereas the AppStore does not.
% The clicks for the AppStore dataset are directly used for computing the relevance-based metrics without the click models, following~\cite{lo2021page,pei2019personalized, ai2018learning}.
The click labels in AppStore dataset are directly used for computing the relevance-based metrics, following~\cite{lo2021page,pei2019personalized, ai2018learning}. Yet the clicks could be biased, and there exist some relevant items that have not been clicked. The list-level approaches tend to place the past-clicked items first, and therefore obtain higher nDCG and MAP. In comparison, the page-level approaches combine information from multiple lists to find relevant items that may have not been clicked to optimize the total utility, and often do not necessarily place clicked items at top positions. Such an observation shows that using past clicks for evaluating may not be able to reflect the true performance for page-level reranking.

% The interleaved arrangement of vertical and horizontal lists on AppStore dataset may lead to a stronger mutual influence of the cross-list.
% \begin{table*}[]
%     % \vspace{-5pt}
%     \caption{Overall performance on AppStore datasets.}
%     % \vspace{-5pt}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|ccccccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{Utility} & \textbf{CTR} & \textbf{CTR\_v} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{ctr\_row4} & \textbf{col\_nDCG} & \textbf{row\_nDCG} & \textbf{col\_MAP} & \textbf{row\_MAP} \\
% \midrule
% INIT & 1.0459 & 1.0571 & 0.2896 & 0.6953 & 0.0391 & 0.0122 & 0.0098 & 0.5774 & 0.6382 & 0.4486 & 0.5237 \\
% miDNN & 1.1704 & 1.1993 & 0.3428 & 0.7588 & 0.0396 & 0.0186 & 0.0107 & 0.5950 & 0.6481 & 0.4680 & 0.5335 \\
% GSF & 1.2183 & 1.1866 & 0.3970 & 0.7505 & 0.0420 & 0.0146 & 0.0142 & 0.5730 & 0.6497 & 0.4429 & 0.5356 \\
% DLCM & 1.3218 & 1.2593 & 0.4521 & 0.8052 & 0.0361 & 0.0176 & 0.0107 & 0.5496 & 0.6418 & 0.4088 & 0.5253 \\
% PRM & 1.3438 & 1.2748 & 0.4497 & 0.8242 & 0.0430 & 0.0151 & 0.0117 & 0.5953 & \textbf{0.6516} & 0.4684 & \textbf{0.5376} \\
% SETRANK & 1.3535 & 1.2938 & 0.4863 & 0.8013 & 0.0366 & 0.0166 & 0.0127 & \textbf{0.5969} & 0.6493 & \textbf{0.4709} & 0.5351 \\
% TRNN & 1.3970 &	1.3641 &	0.5029 &	0.7899 &	0.0431 &	0.0172 &	0.0111 &	0.5904 &	0.6463 &	0.4622 &	0.5310\\
% HMoE &	1.3706 &	1.3744 &	0.5394 &	0.7661 &	0.0414 &	0.0167 &	0.0108 &	0.5935 &	0.6483 &	0.4662 &	0.5338 \\
% DNAHR & 1.4116 & 1.3872 & 0.5312 & 0.8213 & 0.0405 & 0.0107 & 0.0078 & 0.5921 & 0.6410 & 0.4640 & 0.5241 \\
% \textbf{PAR} & \textbf{1.5024*} & \textbf{1.4457*} & \textbf{0.5801*} & \textbf{0.8413*} & \textbf{0.0503} & \textbf{0.0161} & \textbf{0.0146} & 0.5910 & 0.6439 & 0.4631 & 0.5281\\
% \bottomrule
% \end{tabular}
% }
% \footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
%     \label{tab:appstore}
% \end{table*}

% \begin{table*}[]
%     \caption{Overall performance on CTC datasets.}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|cccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{utility} & \textbf{CTR} & \textbf{ctr\_row0} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{nDCG} & \textbf{MAP} \\
% \midrule
% init & 1.2706 & 1.2545 & 0.5030 & 0.3747 & 0.3161 & 0.0607 & 0.4953 & 0.3241 \\
% miDNN & 1.3530 & 1.3305 & 0.5302 & 0.3884 & 0.3439 & 0.0680 & 0.5090 & 0.3415 \\
% GSF & 1.2791 & 1.3252 & 0.5308 & 0.3899 & 0.3386 & 0.0659 & 0.5238 & 0.3618 \\
% DLCM & 1.3494 & 1.3603 & 0.5371 & 0.4064 & 0.3504 & 0.0664 & 0.5303 & 0.3692 \\
% PRM & 1.3722 & 1.3710 & 0.5474 & 0.4014 & 0.3539 & 0.0684 & 0.5212 & 0.3578 \\
% SetRank & 1.3643 & 1.3635 & 0.5432 & 0.4026 & 0.3507 & 0.0671 & 0.5300 & 0.3689 \\
% TRNN & 1.3750 & 1.3602 & 0.5533 & 0.3965 & 0.3430 & 0.0674 & 0.5220 & 0.3587 \\
% HMoE & 1.3615 & 1.3608 & 0.5452 & 0.3968 & 0.3492 & 0.0696 & 0.5236 & 0.3609 \\
% DHANR & 1.3303 & 1.3512 & 0.5382 & 0.3992 & 0.3450 & \textbf{0.0687} & 0.5233 & 0.3597 \\
% \textbf{PAR} & \textbf{1.3963*} & \textbf{1.4016*} & \textbf{0.5648*} & \textbf{0.4153*} & \textbf{0.3540} & 0.0675 & \textbf{0.5463*} & \textbf{0.3897*}\\
% % PAR	1.3963*	1.4016*	0.5648*	0.4153*	0.3540	0.0675	0.5463*	0.3897*
% \bottomrule
% \end{tabular}
% }
% \footnotesize \flushleft\hspace{3cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
% \label{tab:CloudThemeClick}
% \end{table*}


\begin{table*}[]
    \vspace{-10pt}
    \caption{Ablation on AppStore and CTC datasets.}
    \label{tab:ablation}
    \vspace{-10pt}
    \centering
\setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1.2}
% \scalebox{0.86}{
\begin{adjustbox}{max width=0.96\linewidth}
\begin{tabular}{c|ccccccccc|cccccccc}
\toprule
\multirow{2}{*}{\textbf{Variants}} & \multicolumn{9}{c|}{\textbf{AppStore dataset}} & \multicolumn{8}{c}{\textbf{CTC dataset}} \\
\cmidrule{2-18}
& $\mathbf{Utility}$            & $\mathbf{CTR}$             & $\mathbf{CTR_v}$          & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{CTR_{h4}}$         & $\mathbf{nDCG}$            & $\mathbf{MAP}$             & $\mathbf{Utility}$            & $\mathbf{CTR}$             & $\mathbf{CTR_{h1}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h2}}$         & $\mathbf{CTR_{h3}}$         & $\mathbf{nDCG}$             & $\mathbf{MAP}$              \\
\midrule
% PAR-DSA                           & 1.4482          & 1.4236          & 0.5515          & 0.8009          & 0.0432          & 0.0171          & 0.0110          & 0.6292          & 0.5097          & 1.3594          & 1.3712          & 0.5621          & 0.4065          & 0.3399          & 0.0627          & 0.5271           & 0.3648           \\
% PAR-MMoE                           & 1.3950          & 1.4203          & 0.5501          & 0.7997          & 0.0427          & 0.0169          & 0.0108          & \textbf{0.6349}          & \textbf{0.5171} & 1.3821          & 1.3825          & 0.5566          & 0.4106          & 0.3519          & 0.0634          & 0.5321           & 0.3722           \\
% PAR-SSA                            & 1.4595          & 1.4338          & 0.5570          & 0.8083          & 0.0414          & 0.0165          & 0.0105          & 0.6328 & 0.5143          & 1.3757          & 1.3718          & 0.5502          & 0.3978          & \textbf{0.3541} & \textbf{0.0698} & 0.5305           & 0.3688           \\
% PAR-DN      & 1.4743          & 1.4343          & 0.5555          & 0.8076          & 0.0431          & 0.0171          & 0.0110          & 0.6327          & 0.5144          & 1.3146          & 1.3876          & 0.5547          & 0.4109          & 0.3506          & 0.0670          & 0.5378           & 0.3787           \\
% PAR-scale                          & 1.4136          & 1.4356          & 0.5547          & 0.8091          & 0.0436          & \textbf{0.0172} & 0.0109          & 0.6305          & 0.5116          & 1.3871          & 1.3803          & 0.5537          & 0.4096          & 0.3501          & 0.0669          & 0.5367           & 0.3779           \\
% \textbf{PAR}                       & \textbf{1.5024} & \textbf{1.4457} & \textbf{0.5801} & \textbf{0.8413} & \textbf{0.0503} & 0.0161          & \textbf{0.0146} & 0.6333          & 0.5151          & \textbf{1.3963} & \textbf{1.4016} & \textbf{0.5648} & \textbf{0.4153} & 0.3540          & 0.0675          & \textbf{0.5463*} & \textbf{0.3897*}\\
PAR-DSA & 1.4482 & 1.4236 & 0.5515 & 0.8009 & 0.0432 & 0.0171 & 0.0110 & 0.6292 & 0.5097 & 1.3878 & 1.3882 & 0.5493 & 0.4133 & 0.3584 & 0.0673 & 0.5379 & 0.3789 \\
PAR-HDSA & 1.4129 & 1.4193 & 0.5566 & 0.7917 & 0.0431 & \textbf{0.0172} & 0.0108 & 0.6337 & 0.5154 & 1.3629 & 1.3757 & 0.5593 & 0.4113 & 0.3406 & 0.0643 & 0.5334 & 0.3736 \\
PAR-scale    & 1.4136          & 1.4356          & 0.5547          & 0.8091          & 0.0436          & \textbf{0.0172} & 0.0109          & 0.6305          & 0.5116          & 1.3895          & 1.3933          & 0.5589          & 0.4095          & 0.3556          & \textbf{0.0692} & 0.5399          & 0.3816          \\
PAR-SSA      & 1.4595          & 1.4338          & 0.5570          & 0.8083          & 0.0414          & 0.0165          & 0.0105          & 0.6328      & 0.5143          & 1.3885          & 1.3914          & 0.556           & 0.4092          & 0.3586          & 0.0676          & 0.5393          & 0.3809          \\
PAR-DN     & 1.4743          & 1.4343          & 0.5555          & 0.8076          & 0.0431          & 0.0171          & 0.0110          & 0.6327          & 0.5144          & 1.4219          & 1.4026          & 0.5657          & 0.4151          & 0.3552          & 0.0666          & 0.5423          & 0.3848          \\
PAR-MMoE & 1.3950 & 1.4203 & 0.5501 & 0.7997 & 0.0427 & 0.0169 & 0.0108 & \textbf{0.6349} & \textbf{0.5171} & 1.3716 & 1.3751 & 0.5531 & 0.4056 & 0.3484 & 0.068 & 0.5279 & 0.3658\\
\textbf{PAR} & \textbf{1.5024} & \textbf{1.4457} & \textbf{0.5801} & \textbf{0.8413} & \textbf{0.0503} & 0.0161          & \textbf{0.0146} & 0.6333          & 0.5151          & \textbf{1.4446} & \textbf{1.4137} & \textbf{0.5693} & \textbf{0.4174} & \textbf{0.3594} & 0.0677          & \textbf{0.5548*} & \textbf{0.4005*}\\
\bottomrule
\end{tabular}
\end{adjustbox}
% }
\footnotesize \flushleft\hspace{0.3cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best variant.
\vspace{-12pt}
\end{table*}

% \begin{table*}[]
%     % \vspace{-5pt}
%     \caption{Ablation on AppStore dataset.}
%     % \vspace{-5pt}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|ccccccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{utility} & \textbf{CTR} & \textbf{ctr\_col} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{ctr\_row4} & \textbf{col\_nDCG} & \textbf{row\_nDCG} & \textbf{col\_MAP} & \textbf{row\_MAP} \\
% \midrule
% PAR-DSA             & 1.4482           & 1.4236          & 0.5515            & 0.8009             & 0.0432             & 0.0171    & 0.0110             & 0.5843             & 0.6404             & 0.4544            & 0.5235            \\
% PAR-MMoE             & 1.3950           & 1.4203          & 0.5501            & 0.7997             & 0.0427             & 0.0169             & 0.0108             & 0.5836             & \textbf{0.6477}    & 0.4531            & \textbf{0.5331}   \\
% PAR-SSA              & 1.4595           & 1.4338          & 0.5570            & 0.8083             & 0.0414    & 0.0165    & 0.0105             & \textbf{0.5914}    & 0.6431             & \textbf{0.4641}   & 0.5269            \\
% PAR-DN             & 1.4743           & 1.4343          & 0.5555            & 0.8076             & 0.0431             & 0.0171    & 0.0110             & 0.5760             & 0.6469             & 0.4432            & 0.5322            \\
% PAR-scale &	1.4136 &	1.4356 &	0.5547 &	0.8091 &	0.0436 &	\textbf{0.0172} &	0.0109 &	0.5872 &	0.6413 &	0.4586 &	0.5248 \\
% \textbf{PAR}         & \textbf{1.5024}  & \textbf{1.4457} & \textbf{0.5801}   & \textbf{0.8413}    & \textbf{0.0503}    & 0.0161             & \textbf{0.0146}    & 0.5910    & 0.6439             & 0.4631            & 0.5281           \\
% % PAR-DSA & 1.4585 & 1.4279 & 0.5529 & 0.8035 & 0.0432 & \textbf{0.0173} & 0.011 & 0.5903 & 0.6381 & 0.4614 & 0.5205 \\
% % PAR-MMoE & 1.4053 & 1.4217 & 0.5516 & 0.8006 & 0.0421 & 0.0168 & 0.0106 & 0.5829 & \textbf{0.6504} & 0.4520 & \textbf{0.5364} \\
% % PAR-SSA & 1.4448 & 1.4314 & 0.5525 & 0.8070 & 0.0437 & 0.0172 & 0.011 & 0.5908 & 0.6442 & 0.4626 & 0.5287 \\
% % \textbf{PAR} & \textbf{1.5024} & \textbf{1.4457} & \textbf{0.5801} & \textbf{0.8413} & \textbf{0.0503} & 0.0161 & \textbf{0.0146} & \textbf{0.5910} & 0.6439 & \textbf{0.4631} & 0.5281\\
% \bottomrule
% \end{tabular}
% }
% % \footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
%     \label{tab:ablation_appstore}
% \end{table*}

% \begin{table*}[]
%     % \vspace{-5pt}
%     \caption{Ablation on CTC dataset.}
%     % \vspace{-5pt}
%     \centering
% \scalebox{0.89}{
% \begin{tabular}{c|cccccccc}
% \toprule
% \multicolumn{1}{l}{} & \textbf{utility} & \textbf{CTR}    & \textbf{ctr\_row0} & \textbf{ctr\_row1} & \textbf{ctr\_row2} & \textbf{ctr\_row3} & \textbf{nDCG}    & \textbf{MAP}     \\
% \midrule
% PAR-DSA             & 1.3594           & 1.3712          & 0.5621             & 0.4065             & 0.3399             & 0.0627             & 0.5271           & 0.3648           \\
% PAR-MMoE             & 1.3821           & 1.3825          & 0.5566             & 0.4106             & 0.3519             & 0.0634             & 0.5321           & 0.3722           \\
% PAR-SSA              & 1.3757           & 1.3718          & 0.5502             & 0.3978             & \textbf{0.3541}    & \textbf{0.0698}    & 0.5305           & 0.3688           \\
% PAR-DN             & 1.3146           & 1.3876          & 0.5547             & 0.4109             & 0.3506             & 0.0670             & 0.5378           & 0.3787           \\
% PAR-scale &	1.3871 &	1.3803 &	0.5537 &	0.4096 &	0.3501 &	0.0669 &	0.5367 &	0.3779\\
% \textbf{PAR}         & \textbf{1.3963}  & \textbf{1.4016} & \textbf{0.5648}    & \textbf{0.4153}    & 0.3540             & 0.0675             & \textbf{0.5463*} & \textbf{0.3897*}\\
% \bottomrule
% \end{tabular}
% }
% % \footnotesize \flushleft\hspace{0cm} $*$ denotes statistically significant improvement (measured by t-test with $p$-value $<$ 0.05) over the best baseline.
%     \label{tab:ablation_ctc}
% \end{table*}
\vspace{-5pt}
\subsection{In-depth Analysis}

\subsubsection{Ablation study}
To investigate the effectiveness of each component in PAR, we design several variants of PAR and conduct a series of experiments on AppStore and CTC datasets.
\begin{itemize}[leftmargin=10pt]
    \item \textbf{PAR-DSA} replaces the dual-side attention in HDS-Attn with a self-attention, thus removing the user history from the module.
    \item \textbf{PAR-HDSA} removes the HDS-Attn module.
    \item \textbf{PAR-scale} replaces the SS-Attn module with a self-attention.
    \item \textbf{PAR-SSA} removes the SS-Attn module.
    \item \textbf{PAR-DN} removes the dense network.
    \item \textbf{PAR-MMoE} replaces the MMoE module with a single MLP.
\end{itemize}
The comparison of the above variants and the original PAR on AppStore and CTC datasets are presented in Table~\ref{tab:ablation}. Compared to the original PAR, the performances of the variants all decline to some extent, indicating the effectiveness of each module. Among all the variants, PAR-HDSA generally suffered the greatest drop in utility, which suggests that incorporating intra- and inter-list interaction can enhance the performance of page-level reranking. The decline of PAR-DSA indicates the importance of personalized preferences in user behaviors for reranking. Removing the MMoE and SSA modules also introduces a large decrease, illustrating the impact of modeling the differences and commonalities between lists and the page format. There is no significant gap between the results of PAR-SSA and PAR-scale, revealing that it is the distance-aware influence factor that contributes primarily to the SSA module. The basic self-attention is insufficient to model different page formats.



\subsubsection{Case Study}

 \begin{figure}[t]
    \centering
    \vspace{0pt}
    \includegraphics[width=\linewidth]{figures/case-study-2.pdf}
    \vspace{-20pt}
    \caption{
    (a) The attention weights (normalized along the horizontal axis) of the list-level self-attention in HDS-Attn. 
    (b) The pairwise attention weights between the target item (highlighted by a red box) and other items in SS-Attn.}
    \label{fig:case_study}
    \vspace{-13pt}
\end{figure}

To explore the mutual influence between lists and the spatial relationship between items, we select a page from the AppStore and visualize the attention weights from list-level self-attention in HDS-Attn and spatial-scaled attention (SS-Attn). Figure~\ref{fig:case_study}(a) presents the heatmap of the vertical list $v$ and the four horizontal lists $h1$, $h2$, $h3$, and $h4$, with each row being the attention weights of a list. In Figure~\ref{fig:case_study}(a), all lists have a high attention weight for $h1$, probably because $h1$ has the most clicks and can provide more information. List $v$, neighboring all the other lists, receives the next highest number of clicks, and thus the other lists also have a relatively high attention weight for $v$. Conversely, $h2$-$h4$, locating further away with lower CTR, have smaller attention weights. 

As for spatial-scaled attention, we select a target item at the third position of the second horizontal list and then visualize its attention weights on all the items on the F-shape page in Figure~\ref{fig:case_study}(b), from which we observe a general pattern of spatial decay. The target item has the greatest attention weight on itself, and the weights on its surrounding items roughly follow the pattern that the further away the item is, the less weight it gets. Furthermore, we find that there are outliers that violate the spatial decay pattern. In the first horizontal list, the first item $i_1$ and second item $i_2$ have higher attention weights (0.0149 and 0.0150) than the third item $i_3$ (0.0148), though $i_3$ is closer to the target item. The possible reason is that $i_1$ and $i_2$ share the same category with the target item (they are all short-video apps), while $i_3$ is a search engine app. The similar category promotes the pairwise mutual influence between items. As such, we conclude that the SS-Attn can automatically learn the combination of the spatial effect and the pairwise influence.


% First, there is a pattern of spatial decay. The target item has the greatest attention weight on itself, and the weights on its surrounding items roughly follow the pattern that the further away the item is, the less weight it gets. 
% Second, there are outliers that violate the spatial decay pattern. In the first horizontal list, the first item $i_1$ and second item $i_2$ have higher attention weights (0.0149 and 0.0150) than the third item $i_3$ (0.0148), though $i_3$ is closer to the target item. The possible reason is that $i_1$ and $i_2$ share the same category with the target item (i.e., short-video app), while $i_3$ is a search engine app. The similar category promotes the pairwise mutual influence between items.
% Second, the weights of the bottom items are usually greater than those of the top items, which is inconsistent with the common cascade assumption. This may be attributed to the fact that the item that the user focuses on is usually swept to the upper part of the phone screen, making it easier for the user to compare the target item with the bottom items.


\vspace{-5pt}
\section{Related Works}\label{sect:related}

% We review studies on (1) reranking, (2) multi-scenario recommendation, and (3) whole-page optimization.

\subsection{Reranking}

% According to the input and context, the reranking methods can be divided into (\romannumeral1) list-level reranking, and (\romannumeral2) page-level reranking.

Most existing reranking methods are list-level, and conduct reranking separately for each individual list \cite{feng2021grn,xi2021context,ai2018learning,bello2018seq2slate,feng2021revisit,pang2020setrank,pei2019personalized}. Various network structures have been applied for modeling the mutual influences within the list. For example, miDNN~\cite{zhuang2018globally} uses DNN with global feature extension to capture mutual influences between items. A group-wise scoring function (GSF)~\cite{ai2019learning} is learned by enumerating all the feasible item permutations of the list. DLCM~\cite{ai2018learning} employs the gated recurrent unit (GRU) to encode the whole ranking list into the item representations. PRM~\cite{pei2019personalized} and SetRank~\cite{pang2020setrank} adopt the self-attention mechanism to model the influence between any pair of items in the list. Yet the performance of list-level reranking algorithms is usually suboptimal when the recommendation page presented to the user is in a multi-list style.

\citet{hao2021re} find the information from other lists on the page can improve the performance of reranking, and propose a deep and hierarchical attention network reranking (DHANR) model. They aggregate the page-wise context into a static page representation vector, and apply an identical list-level reranking algorithm for all the lists with the page representation as shared side information. However, DHANR fails to capture the dynamic page-level interaction between items, and is insensitive to the different page formats or the commonalities and distinctions between lists. Our proposed PAR fully exploits the page-wise context and captures multifaceted fine-grained item influences across lists.

\vspace{-7pt}
\subsection{Multi-scenario Learning to Rank}
Multi-scenario learning to rank aims to improve the overall performance in different scenarios, which can be generally classified into two categories: (1) multi-task learning (MTL) \cite{chen2020scenario,li2020improving,gu2021self,sheng2021one,zhao2019recommending}, and (2) multi-agent reinforcement learning (MARL) \cite{feng2018learning,he2020learning}.
MTL-based methods formulate the ranking problems from different scenarios as different tasks, and devise a single model to solve the multiple tasks simultaneously. For instance, HMoE~\cite{li2020improving} utilizes Multi-task Mixture-of-Experts~\cite{ma2018modeling,zhao2019recommending} to identify the commonalities and distinctions between scenarios implicitly. As for MARL-based methods~\cite{feng2018learning,he2020learning}, each scenario has a local ranking agent, and the agents are trained collaboratively to improve the overall performance. However, the agents are updated in an online setting with instant feedback, which is different from ours.

Page-level reranking intends to simultaneously rerank lists on the same page, which emphasizes on user behaviors when examining a recommendation page as a whole. How to model the page format and contexts is key to page-level reranking, which is ignored in multi-scenario learning to rank. 
% Still, the problem of page-level reranking and multi-scenario learning to rank have some common characteristics, and could be compensated for each other.
%  Different scenarios in the multi-scenario learning to rank are often not on the same page. 
% STAR~\cite{sheng2021one} designs a topologically shared model structure for the multi-scenario ranking. 
\vspace{-7pt}
\subsection{Whole-page Optimization}
Whole-page optimization focuses on improving the display of the recommendation page, which generally falls into two categories. 

The first category~\cite{wang2016beyond,wang2018optimizing,hill2017efficient,wang2017efficient,xiao2022tile,zhao2018deep,oosterhuis2018ranking} aims to find the optimal presentation style for each item on the page. Presentation style includes positions, image sizes, text fonts, etc. The problem is then formulated as a combinatorial optimization problem of determining positions and other presentation styles for each item, where graph matching~\cite{wang2016beyond,wang2018optimizing}, bandit~\cite{hill2017efficient,wang2017efficient} or reinforcement learning (RL)~\cite{wang2018optimizing,xiao2022tile,zhao2018deep,oosterhuis2018ranking} algorithms are proposed. This type of method, however, is designed for mapping one single initial list into a 2D geometrical layout, which is different from our work --- the input of PAR is multiple initial lists of different themes.

The second category~\cite{gomez2015netflix,bendada2020carousel,ding2019whole,lo2021page} is designed to select and rank the widgets (list of items) of the page. 
% Given a set of fixed ordered widgets, these methods try to select personalized themes of widgets to meet users' needs. 
Given a set of widgets where the order of items for each widget is fixed, these methods try to select personalized themes of widgets to meet users' needs. 
These models, though involving the page-level information, is not the focus of our work. In this work, we jointly optimize the arrangement of items for multiple lists by considering the page-wise context.

% focuses on the problem of whole-page optimization by selecting and ranking the widgets. Each widget is constructed in a list format. Nevertheless, they do not rerank the items in each widget list (i.e., the content of the widget is fixed). Hence, they reduce the whole-page optimization to a widget-ranking problem, where we can simply adopt traditional list-level reranking algorithms by regarding each widget as a large ``item''. These methods are incompatible with the page-level reranking problem, where we seek to arrange fine-grained reranking of items within each widget. 

% optimal content and presentation format for each widget (e.g., button, image, text, list of URLs) in the page. 
% The widget does not necessarily be constructed in list format (e.g., button, image, text, list of URL). Therefore, they reduce the whole-page optimization to a combinatorial optimization problem, 
% However, these methods are unsuitable for page-level reranking by regarding each list as a widget due to the following reasons. 
% (1) They requires each widget to have limited number of variants. One list that contains $m$ items can have $m!$ variants, causing the combinatorial explosion problem.
% (2) Most of these methods are online algorithms, and requires real-time interaction with users. This violates the offline paradigm in the traditional reranking setting where we seek to construct the reranker offline to avoid hurting the user experience.





% In this work, we focus on the page-level reranking, which is fairly different from previous whole-page optimization methods mentioned above. The goal of page-level reranking is to rerank the item within each list by considering the page-wise context (e.g., the content of other lists, the page format). 



